A Review of Incorporating Psychological Theories in LLMs

Psychological insights have long shaped pivotal NLP breakthroughs, from attention mechanisms to reinforcement learning and social modeling. As Large Language Models (LLMs) develop, there is a rising consensus that psychology is essential for capturing human-like cognition, behavior, and interaction. This paper reviews how psychological theories can inform and enhance stages of LLM development. Our review integrates insights from six subfields of psychology, including cognitive, developmental, behavioral, social, personality psychology, and psycholinguistics. With stage-wise analysis, we highlight current trends and gaps in how psychological theories are applied. By examining both cross-domain connections and points of tension, we aim to bridge disciplinary divides and promote more thoughtful integration of psychology into NLP research.

==> application/application_agent.tex <==
\sara{The following are from applications of personality psych.}

\subsubsection{Modeling Personality in Dialogue}
\textbf{Dialogue Understanding}

Personality traits shape dialogue interactions in LLMs, influencing negotiation and persona-based modeling \cite{huang-hadfi-2024-personality, cheng-etal-2023-marked}. \cite{huang-hadfi-2024-personality} simulated LLM agents with Big Five traits, showing that agreeableness led to better negotiation outcomes while neuroticism resulted in worse ones. \cite{cheng-etal-2023-marked} introduced \textbf{Marked Personas}, revealing biases in LLM-generated personas using a prompt-based method. Their findings highlight concerns over stereotyping in AI-driven dialogue. Future work should refine personality modeling while mitigating biases.

\textbf{Dialogue Generation}

Recent studies have advanced personality-aware dialogue generation by moving beyond static personas, incorporating multimodal empathy, and improving persona consistency \cite{pal-etal-2025-beyond, wu-etal-2025-traits, takayama-etal-2025-persona, chen-etal-2025-comif, ye-etal-2025-sweetiechat}.

\cite{pal-etal-2025-beyond} introduced a dataset of 400K dialogues based on clustered Reddit journal entries, enhancing personality modeling by capturing Big Five traits in generated dialogues. \cite{wu-etal-2025-traits} incorporated multimodal cues (text and images) to generate empathetic responses tailored to user personality. \cite{takayama-etal-2025-persona} improved persona consistency in dialogues using \textbf{Pseudo Preference Tuning}, generating more coherent responses via Direct Preference Optimization (DPO). \cite{chen-etal-2025-comif} proposed \textbf{CoMIF}, a framework that models multiple interaction factors (e.g., personality, emotion, topic) to enhance dialogue realism. \cite{ye-etal-2025-sweetiechat} developed a strategy-enhanced role-playing framework for emotional support agents, refining dialogue adaptation across diverse scenarios.

These approaches push dialogue generation toward more natural, context-aware, and personality-consistent interactions, but challenges remain in balancing multiple personality factors and improving long-term consistency.

\subsubsection{Building Agents with Persona}
\textbf{Dialogue Agents}

Recent work explores persona-driven dialogue agents, focusing on argument generation and personality-based synthetic dialogues \cite{hu-etal-2025-debate, han-etal-2024-psydial}.

\cite{hu-etal-2025-debate} proposed a \textbf{persona-driven multi-agent framework} for argument generation, where agents debate from distinct perspectives to collaboratively construct coherent narratives. This method enhances output diversity and reasoning depth. \cite{han-etal-2024-psydial} introduced \textbf{PSYDIAL}, a personality-based dialogue dataset emphasizing Extraversion from the Big Five model. Their approach improves personality expression in chatbot responses compared to standard models.

These studies highlight the potential of persona-driven frameworks in enhancing dialogue diversity, coherence, and personality alignment.

\textbf{Role-Play Agents}

Recent work has focused on role-playing LLM agents, evaluating their persona alignment, social interaction, and ability to simulate diverse perspectives \cite{castricato-etal-2025-persona, wu-etal-2025-raiden, wang-etal-2025-decoding, chen-etal-2024-socialbench, wang-etal-2024-rolellm, wang-etal-2024-characteristic, mahajan-shaikh-2024-persona, gong2024creamcomparisonbasedreferencefreeeloranked}.

\cite{castricato-etal-2025-persona} introduced \textbf{PERSONA}, a testbed for pluralistic alignment, using 1,586 synthetic personas to evaluate LM responses across diverse user profiles. \cite{wu-etal-2025-raiden} developed the \textbf{RAIDEN Benchmark}, a large-scale dataset assessing role-playing conversational agents (RPCAs) with 40K multi-turn dialogues. \cite{wang-etal-2025-decoding} simulated social opinion networks, modeling echo chambers and polarization using LLM agents. \cite{chen-etal-2024-socialbench} proposed \textbf{SocialBench}, the first benchmark evaluating role-playing agents’ social intelligence at both individual and group levels.

Further, \cite{wang-etal-2024-rolellm} introduced \textbf{RoleLLM}, a framework for benchmarking and fine-tuning role-playing abilities, creating RoleLLaMA and RoleGLM. \cite{wang-etal-2024-characteristic} developed \textbf{Character100}, a dataset for simulating real-life personas in AI agents, enabling systematic evaluation. \cite{mahajan-shaikh-2024-persona} proposed a persona-aware heterogeneous graph transformer to improve response generation in multi-party conversations.

These efforts advance role-playing agents by improving persona consistency, diversity, and realism, though challenges remain in balancing adaptability with coherence in long-term interactions.

\textbf{Improve LLMs through persona}
\sara{discuss again where this belong}

Personality has been used to enhance LLMs in persona consistency, self-improvement, truthfulness, and dialogue coherence.
\cite{jiang-etal-2024-personallm} introduced \textbf{PersonaLLM}, showing that LLMs can generate stable Big Five personality traits, with human evaluators recognizing them with 80\% accuracy. \cite{zhang-etal-2024-self-contrast} proposed \textbf{Self-Contrast}, a method improving LLM reflection by identifying inconsistencies, enhancing response stability. \cite{joshi-etal-2024-personas} introduced the \textbf{Persona Hypothesis}, suggesting LLMs encode truthful and untruthful personas from pretraining data, influencing their truthfulness. \cite{kim-etal-2024-panda} tackled the \textbf{persona overuse problem} in dialogue, developing \textbf{PANDA} to mitigate excessive persona attribution.

\subsubsection{Measuring Personality}

\textbf{Measuring User Personality}

NLP research increasingly explores LLMs' ability to infer user personality from text, moving beyond structured psychological tests \cite{rao-etal-2023-chatgpt, yang-etal-2023-psycot} to interactive and multi-agent frameworks \cite{yang-etal-2024-psychogat, yeo-etal-2025-pado}. \cite{rao-etal-2023-chatgpt} developed an MBTI-based evaluation framework, while \cite{yang-etal-2023-psycot} improved Big Five assessments using psychological questionnaire-inspired \textit{Chain-of-Thought} (CoT) prompting. More recent work includes \textbf{PsychoGAT} \cite{yang-etal-2024-psychogat}, which gamifies personality assessments, and \textbf{PADO} \cite{yeo-etal-2025-pado}, a multi-agent framework enhancing contextual inference. Challenges remain in ensuring interpretability, reliability, and applicability across diverse populations, highlighting the need for deeper psychological integration in LLM-driven personality assessment.

\textbf{Measuring Personality Consistency}

Research on personality consistency in LLMs examines whether traits remain stable across interactions and contexts \cite{frisch-giulianelli-2024-llm, amidei-etal-2025-exploring}. \cite{frisch-giulianelli-2024-llm} found that LLMs conditioned on asymmetric personality profiles exhibit varying degrees of consistency in dialogue, highlighting challenges in maintaining stable traits. \cite{amidei-etal-2025-exploring} showed that language switching weakly but significantly alters GPT-4o’s personality expression, reflecting cultural stereotypes. These studies highlight the need for improving personality stability and mitigating biases in LLM-driven interactions.

\textbf{Measuring Machine Personality}
\sara{should this go into interpretability????}

Research on machine personality explores whether LLMs exhibit stable traits and how these can be modified \cite{10.1007/978-981-97-9434-8_19, hu-collier-2024-quantifying}. \cite{10.1007/978-981-97-9434-8_19} introduced \textbf{PersonalityEdit}, a benchmark for systematically adjusting LLM responses to align with \textit{Neuroticism, Extraversion, and Agreeableness}, highlighting challenges in maintaining consistency. \cite{hu-collier-2024-quantifying} examined the \textbf{Persona Effect}, showing that while persona-based prompting improves annotations in ambiguous cases, its impact is limited in most subjective NLP datasets. Future research should refine personality control mechanisms and assess their impact on human-LLM interactions.

While research on human personality assessment using LLMs has gained traction, a parallel line of work explores whether and how personality traits manifest within LLMs themselves. Current studies primarily focus on two areas: \textit{(1) Editing or modifying personality traits in LLMs} to control their responses and \textit{(2) Evaluating the influence of persona-related variables} on LLM behavior \cite{10.1007/978-981-97-9434-8_19, hu-collier-2024-quantifying}.

==> application/application_dep.tex <==
\lin{I will refactor the following sections (7.0.1-7.0.4) by types of applications.}

\subsubsection{Dual-Process Models}
\label{subsubsec:dual_process}
Dual-process models, which separate fast, intuitive from slow, deliberate reasoning, offer a promising framework for enhancing LLM performance. For instance, chain-of-thought prompting \cite{wei2022chain} encourages the model to generate intermediate reasoning steps, effectively engaging System 2 processes and improving performance on complex tasks. Building on this, the DynaThink framework \cite{pan-etal-2024-dynathink} enables LLMs to dynamically select between rapid and thorough inference based on task complexity. Additionally, the Tree of Thoughts approach \cite{yao2024tree} allows the exploration of multiple reasoning paths concurrently, further refining deliberative processing. Together, these methods not only reduce errors and enhance decision-making but also open avenues for future research, such as integrating reinforcement learning for dynamic task routing and improving long-horizon context management.

\subsubsection{ToM}
\label{subsubsec:tom}
Integrating ToM into LLMs enhances their ability to infer beliefs, desires, and intentions, crucial for social interaction \cite{baron1985does}. Recent research focuses on two areas: \textbf{(1)} evaluation and benchmarking, and \textbf{(2)} model enhancements for interpersonal and multi-agent interactions.

For evaluation, benchmarks like \textit{ToMBENCH} \cite{chen-etal-2024-tombench} and \textit{OpenToM} \cite{xu-etal-2024-opentom} assess LLMs on mental state modeling, while \textit{HI-TOM} \cite{wu-etal-2023-hi} and \textit{FANTOM} \cite{kim-etal-2023-fantom} test higher-order reasoning and asymmetric information scenarios. \citet{soubki-etal-2024-views} extend ToM evaluation to spoken dialogues, highlighting gaps between LLM and human performance. Surveys \cite{ma-etal-2023-towards-holistic, sap-etal-2022-neural} outline existing challenges and research directions.

For model enhancements, \textbf{interpersonal methods} improve missing knowledge inference \cite{bortoletto-etal-2024-limits}, common ground alignment \cite{qiu-etal-2024-minddial}, and cognitive modeling \cite{wu-etal-2024-coke}. \textbf{Multi-agent approaches} enable characters' belief tracking \cite{sclar-etal-2023-minding} and coordination in social tasks \cite{wang2021tomc, sclar2022symmetric}. Logic-based frameworks \cite{sileo-lernould-2023-mindgames} show that increasing model scale does not always enhance epistemic reasoning. Inspired by dual-process and Simulation Theory, strategies \cite{wilf-etal-2024-think, jung-etal-2024-perceptions} refine ToM capabilities through task decomposition, further extended by recursive simulations \cite{sarangi-etal-2025-decompose}.

\subsubsection{Persuasion Models}
\label{subsubsec:persuasion}
Persuasion models provide insights into shaping language and behavior to influence attitudes and decisions. In \textbf{interpersonal interactions}, studies have developed persuasive chatbots and recommender systems. \citet{gollapalli-ng-2025-pirsuader} employ a persuasive dialog act schema and reinforcement learning to mitigate psychological insulin resistance, while \citet{furumai-etal-2024-zero} integrate LLM-generated strategies with retrieval to enhance factuality and persuasiveness. Similarly, \citet{qin-etal-2024-beyond} and \citet{jin-etal-2024-persuading} guide explanation generation using credibility-aware strategies and intent-to-strategy reasoning. \citet{zeng-etal-2024-johnny} take a different approach, applying a persuasion taxonomy to generate adversarial prompts, exposing LLM vulnerabilities.

In \textbf{multi-agent settings}, persuasion models facilitate negotiation and debate simulations. \citet{huang-hadfi-2024-personality} use synthesized personality traits to model LLM-based negotiations, mirroring human behaviors. \citet{10.5555/3692070.3693020} demonstrate that structured debates between LLM experts improve truthfulness, while \citet{rescala-etal-2024-language} extend datasets to assess argument strength, with ensemble models outperforming human evaluation.

These studies show advancements in persuasive effectiveness, credibility, and negotiation alignment, but challenges remain, such as long-horizon context management and jailbreak risks. Future directions include integrating reinforcement learning and multi-domain datasets to enhance LLMs' social influence capabilities.

\subsubsection{Self-Reflective Mechanisms}
\label{subsubsec:self_reflect}
Self-reflective methods have been applied across various tasks, including hallucination mitigation and factuality improvement \cite{ji-etal-2023-towards}, machine translation \cite{chen-etal-2024-dual, wang-etal-2024-taste}, question answering \cite{li-etal-2024-hindsight, zhang-etal-2024-learn, kassner-etal-2023-language}, mathematical reasoning \cite{zhang-etal-2024-learn}, and named entity recognition \cite{heng-etal-2024-proggen}. \textbf{Multi-agent frameworks}, such as reflective collaboration \cite{NEURIPS2024_fa54b0ed} and hierarchical agents \cite{pmlr-v235-du24h}, extend these techniques to collective environments.

Several methods adopt dual or multi-step reflection processes \cite{li-etal-2024-think}, where iterative self-reflection \cite{ji-etal-2023-towards, yan-etal-2024-mirror} and task decomposition \cite{wang-etal-2024-taste, zhang-etal-2024-self-contrast} refine intermediate reasoning steps, improving factuality and reducing hallucinations. Reinforcement learning (RL) further optimizes self-reflection, as seen in reflection-reinforced self-training \cite{dou-etal-2024-rest}, confidence-calibrating reward functions \cite{xu-etal-2024-sayself}, and semantic memory-augmented RL \cite{gupta-etal-2024-metareflection}, which enhance task performance. Additionally, self-reflective rationales \cite{kassner-etal-2023-language, ramnath2024tailoring} and uncertainty-aware methods \cite{zhao-etal-2024-fact, NEURIPS2024_b130a569} help calibrate confidence levels, though studies indicate that LLM self-explanations are not always reliable \cite{madsen-etal-2024-self}.

These methods collectively demonstrate that self-reflection can improve consistency, reasoning, and calibration across diverse tasks. While their connection to self and identity theories is indirect, they align with the core idea that introspection and self-assessment drive continuous improvement. Future research should explore unified frameworks that integrate these techniques and more explicitly align them with self and identity constructs, potentially enabling LLMs to exhibit more human-like behaviors and understand social norms and nuances. Additionally, theories such as self-identity, self-discrepancy, and self-affirmation present promising avenues for enhancing LLMs’ ability to model human behavior and complex social interactions.

==> behavioral/behavioral.tex <==
\subsection{Observational Learning}
Observational learning, as introduced by \citet{bandura1977social}, posits that individuals can learn complex behaviors simply by observing others. Within Large Language Models (LLMs), this concept is loosely paralleled by the way these models “observe” large corpora of text to internalize patterns of language. The key difference between human learning and machine learning goes beyond the amount of data and resources required; it also relates to the nature versus nurture debate. Humans are born with innate representations of language and knowledge, while language models must learn everything from data. This raises the challenge of how LLMs can approximate these inherent structures without the built-in cognitive frameworks that humans possess.

\subsubsection{Core Theoretical Foundation}
\citet{bandura1977social, bandura1986social} highlighted four key components of observational learning: attention, retention, reproduction, and motivation. Although LLMs do not replicate human cognitive processes, advancements in LLM architectures have been heavily influenced by these ideas, and thus these components have conceptual analogs in model training:

\begin{itemize}
    \item \textbf{Attention}: Transformers \cite{vaswani2017attention} use attention mechanisms to focus on specific parts of input text, mirroring how learners focus on relevant aspects of observed behavior.
    \item \textbf{Retention}: Through the training objective (predicting tokens in a sequence), LLMs encode and store language patterns in their model parameters \cite{devlin2018bert, liu2019roberta}.
    \item \textbf{Reproduction}: At inference time, LLMs “reproduce” the patterns learned during training by generating text sequences that reflect the statistical regularities in the data \cite{radford2018improving, brown2020language}.
    \item \textbf{Motivation}: While LLMs do not possess intrinsic motivation in the psychological sense, the optimization of the training objective serves as a proxy, pushing the model to “imitate” patterns that minimize loss.
\end{itemize}

This mapping between Bandura’s framework and LLM operations underlines how deep learning architectures can be viewed as a “computational lens” on observational learning. Yet unlike humans—who may have innate linguistic predispositions—LLMs rely solely on patterns drawn from large-scale text, raising questions about whether current model architectures can capture the depth and flexibility of human cognition.

\subsubsection{Scale and Diversity in Observed Data}
A defining characteristic of LLMs is the sheer volume and diversity of text data they ingest, spanning websites, books, social media, and more. This expansive coverage allows models to acquire a broad range of linguistic styles and domain knowledge. From an observational learning standpoint, the larger and more diverse the “demonstrations” (i.e., text corpora) the model witnesses, the richer its learned representations can become \cite{lecun2015deep}. However, the difference in “nature vs. nurture” is stark: humans start with certain cognitive scaffolds, whereas models must approximate those structures from raw inputs alone.

\subsubsection{Ethical and Practical Implications}
As data size and model capacity increase, LLMs become more adept at few-shot and zero-shot tasks \cite{kalyan2024survey}. However, such large-scale “observation” can also ingest harmful biases \cite{bender2021dangers, ai2024defending} and factual inaccuracies \cite{xu-etal-2024-earth}. Funny enough, humans also “learn” bias from their environment through observational learning, albeit on a smaller scale. To address similar concerns in LLMs, a common solution involves fine-tuning with human feedback \cite{ouyang2022training} to align model outputs with desired norms. Yet, this approach remains an imperfect fix, partly because LLMs lack the innate moral or cognitive frameworks that guide humans to scrutinize and sometimes reject biased behaviors. As LLMs become more pervasive, these gaps between artificial and human observational learning underscore the importance of carefully curating training data and introducing robust post-training alignment methods.

\subsection{Operant Conditioning \& Reinforcement (Skinner’s Theory)}


Operant Conditioning, a concept pioneered by \citet{skinner1963operant}, posits that behaviors are shaped and maintained by the consequences they produce, specifically through rewards (positive reinforcement) or punishments (negative reinforcement/punishment). In the context of LLMs, Reinforcement Learning from Human Feedback (RLHF) emerges as a direct analog: models are “rewarded” or “penalized” based on how well their generated text aligns with human preferences. This section explores the theoretical foundations and recent empirical work (2022–2024) demonstrating how RLHF applies Skinner’s principles to create more aligned, coherent, and helpful language models.

\subsubsection{Core Theoretical Foundation}
\citet{skinner1963operant}'s foundational text introduced the idea that behavior can be systematically modified through a reinforcement schedule: rewards increase the likelihood of a behavior reoccurring, whereas punishments or a lack of reward diminish it. In his later work \cite{skinner1957behavior}, Skinner applied operant conditioning principles to language acquisition. Although LLMs lack human cognition and experiential learning, RLHF effectively operationalizes Skinner's core insight: Language output shaped by reward signals (from human evaluators) tends to be reproduced by the model in future generations.

\subsubsection{Reinforcement Learning from Human Feedback (RLHF)}
RLHF modifies an LLM’s behavior by collecting human judgments on model outputs, training a reward model to reflect these judgments, and then optimizing the LLM (via a reinforcement learning algorithm) to produce outputs that maximize the learned reward \cite{ziegler2019fine, ouyang2022training}.

\textcolor{red}{temp recent paper}

\iffalse
\paragraph{Back to Basics \cite{ahmadian-etal-2024-back}}
A return to simple REINFORCE methods suggests that highly complex strategies (e.g., PPO, DPO) are not always necessary for effective LLM alignment. While REINFORCE can lower computation costs, the authors emphasize careful tuning of learning rates and entropy terms to handle nuanced user preferences.

\paragraph{RLAIF vs. RLHF \cite{10.5555/3692070.3693141}.}
This work compares purely human-labeled RLHF with AI-assisted feedback (RLAIF), highlighting the cost savings of delegating preference annotations to a secondary model. However, it also warns of potential bias amplification if the AI feedback model is not sufficiently robust.


\paragraph{Aligning Large Multimodal Models with Factually Augmented RLHF \cite{sun-etal-2024-aligning}}
Here, a fact-checking layer is integrated into the RLHF pipeline for image-text tasks, reducing hallucinations in domains like visual question answering.

\paragraph{Direct Large Language Model Alignment Through Self-Rewarding Contrastive Prompt Distillation \cite{liu-etal-2024-direct}}
In this approach, the model generates candidate outputs and self-assesses them via contrastive prompts, minimizing the need for external human feedback. However, such self-rewarding pipelines may overlook subtle, human-specific preferences that are difficult for the model to infer purely from data.
\fi

Inspired by the principles of operant conditioning in behavioral psychology—where rewards reinforce desirable behavior and punishments deter undesirable actions—a return to simpler reinforcement learning methods suggests that highly complex approaches such as PPO or DPO may not be essential for effective large language model alignment. Just as Skinner’s work demonstrated that behavior is modulated by reinforcement schedules, careful tuning of learning rates and entropy terms can capture nuanced user preferences in a similarly systematic manner \cite{ahmadian-etal-2024-back}. In parallel, the comparison between conventional human-labeled feedback and AI-assisted annotation echoes differential reinforcement strategies: delegating preference labeling to a secondary model can yield significant cost savings, yet, like an imbalanced reinforcement schedule, it risks amplifying bias if the auxiliary model is not robust enough \cite{10.5555/3692070.3693141}. Extending this paradigm, incorporating a fact-checking layer within the RLHF pipeline for multimodal tasks—akin to introducing corrective feedback—effectively reduces hallucinations in image-text scenarios such as visual question answering \cite{sun-etal-2024-aligning}. Meanwhile, a self-rewarding approach, where the model generates candidate outputs and self-assesses them via contrastive prompts, minimizes the need for external human intervention, mirroring the concept of intrinsic motivation; however, this method may overlook subtle, human-specific preferences that remain challenging to infer purely from data \cite{liu-etal-2024-direct}.

\bigskip
\noindent
Overall, applying Skinner’s operant conditioning to LLMs illuminates both the promise and limitations of reward-based learning in artificial agents. Although RLHF can significantly improve model alignment, it also underscores the distinction between human and machine learning. Humans innately calibrate their language use through complex social and cognitive cues—internal drives that do not exist in LLMs. In turn, designers of RLHF pipelines must continuously refine their reinforcement signals to approximate these innate, human-centric processes.


==> cog_dev_papers/cog_dev.tex <==
\subsection{Perception}
% \label{subsec:perception}
Perception in psychology encompasses a variety of mechanisms, including bottom-up (data-driven) and top-down (knowledge-driven) processes, selective attention, and subliminal perception---where stimuli below the threshold of conscious awareness can still influence thoughts and behaviors \cite{gregory_topdown_bottomup, greenwald1995subliminel}. Key theories in this domain include:

\begin{itemize}[nosep,topsep=0pt]
    \item \textbf{Top-down/Bottom-up Models:} Suggest that perception arises from both data-driven inputs and higher-level cognitive processes \cite{gregory_topdown_bottomup}.
    \item \textbf{Selective Attention:} Highlights how individuals focus on certain stimuli while filtering out others \cite{treisman1969selective_attention}.
    \item \textbf{Subliminal Perception:} Explores how unconscious stimuli can affect thoughts and behaviors \cite{greenwald1995subliminel}.
\end{itemize}

\subsubsection{Top-Down and Bottom-Up Synergy in LLMs}
Research on LLM perception often explores how top-down and bottom-up processes work together to enhance text understanding.
\citet{rawte2022tdlr} introduce a framework that prioritizes high-level semantic information before dealing with lower-level syntax, which mirrors top-down processing in human perception, where prior knowledge shapes how we interpret incoming details. 
\citet{10.5555/3600270.3601883} show that prompting LLMs with “Let’s think step by step” triggers a similar top-down reasoning style. 
Meanwhile, \citet{araujo-etal-2021-augmenting} adopt predictive coding principles by introducing explicit top-down connections in BERT-style models, allowing the system to anticipate future sentences and adjust its internal representations accordingly. 
\citet{pang-etal-2023-long} combine bottom-up encoding with top-down corrections to capture both granular details and overarching context, reflecting how humans integrate local cues into a global perceptual framework. 
Finally, \citet{zhang-etal-2024-holistic} propose Holistic Automated Red Teaming using a top-down approach for test case generation and multi-turn probing, echoing the psychological idea that higher-level strategies can steer how specific inputs are perceived and evaluated.

\subsubsection{Selective Perception}
\label{subsubsec:selective_perception}
Selective attention and perception are also vital elements in human cognition. 
\citet{maharaj-etal-2023-eyes} highlight selective attention by examining users’ gaze behavior for detecting hallucinations, showing how focusing on high-value cues helps manage complex data. 
\citet{nottingham-etal-2024-selective} applies selective perception by training a small model to filter out irrelevant input, thus aligning with the psychological principle that not all stimuli are processed equally. 
Lastly, \citet{jung-etal-2024-perceptions} explore “perceptions to beliefs” as precursors to theory of mind, illustrating how LLMs process initial sensory or textual cues and then infer hidden mental states---a step that parallels how humans form beliefs from raw perceptual data \cite{baron1985does}.
\paragraph{}
Collectively, these studies highlight the importance of integrating psychological theories of perception into LLM architectures. On one hand, top-down mechanisms can guide models to make better sense of complex inputs, but they risk overreliance on prior assumptions. On the other hand, bottom-up signals and selective attention ensure that new or salient details are not overlooked. While current methods show promise in reducing hallucinations and refining context integration, open challenges remain—such as designing more nuanced subliminal or partial cues for LLMs, and balancing global consistency with local sensitivity. Future work may explore how these perceptual frameworks scale to longer contexts or multimodal inputs, and how combining predictive coding with advanced attention mechanisms might yield even more human-like text understanding.
\subsection{Memory}
\label{subsec:memory}
In psychology, memory is often divided into three stages: encoding (taking in information), storage (maintaining it over time), and retrieval (accessing it when needed) \cite{memory_stage_theory}. The concept of working memory also highlights how individuals hold and manipulate information over the short term \cite{baddeley1974working}. Major theories include:
\begin{itemize}[nosep,topsep=0pt]
    \item \textbf{Multi-Store Model:} Proposes separate short-term and long-term memory stores, each serving different roles in information retention \citep{memory_stage_theory}.
    \item \textbf{Episodic Memory:} Focuses on personal experiences encoded and retrieved with a sense of time and place \citep{tulving1972episodic}.
    \item \textbf{Working Memory:} Emphasizes the short-term holding and manipulation of data during complex tasks \citep{baddeley1974working}.
    \item \textbf{Schema Theory:} Suggests knowledge is structured in layered frameworks that guide interpretation and learning \citep{bartlett1995remembering}.
\end{itemize}

\subsubsection{Memory Mechanisms in LLMs}
Researchers have begun to align these memory concepts with language model architectures. For instance, \citet{kang2024think} extend Decision Transformers with a working memory module, mirroring how humans store information “in mind” briefly when performing tasks. Building on the multi-store approach, \citet{park2024memoria} separate memory into short-term and long-term components to handle catastrophic forgetting, while \citet{liu-etal-2022-incremental} introduce episodic memory prompts that allow knowledge to carry over from one session to the next, recalling how humans preserve task-specific memories through repeated contexts. 

\subsubsection{Episodic and Neuromorphic Retrieval}
Beyond short-term storage, several studies emphasize the role of episodic memory in generating more human-like responses. \citet{miao-etal-2024-episodic} propose a neuromorphic mechanism akin to hippocampal retrieval \citep{wilson1994reactivation} for commonsense counterfactual generation, reflecting how people rely on personal experiences to evaluate new scenarios. \citet{zeng-etal-2024-memorize} propose incremental memory with decremental chunking to efficiently handle large volumes of text in a single pass, paralleling the chunk-based strategies people use to cope with extensive information \citep{miller1956magicalchunking}.

\subsubsection{Random Access and Working Memory Limits}
Moving from sequential to non-sequential memory use, \citet{zhu-etal-2024-beyond} address the challenge of random memory access, suggesting that techniques like recitation can improve a model’s ability to retrieve arbitrary stored elements. Meanwhile, \citet{zhang-etal-2024-working} evaluate LLMs using n-back tasks, a standard measure of working memory capacity in cognitive psychology \citep{baddeley1974working}, revealing inherent reasoning limits even in larger models. \citet{wang-etal-2024-symbolic} and \citet{chi-etal-2023-transformer} adopt symbolic and adaptive-depth methods, respectively, showing how more explicit working memory structures can enhance rule-based reasoning and extrapolation to longer sequences. \citet{li-etal-2023-large} focus on controllable working memory that balances an LLM’s internal knowledge with context provided at inference time, bridging ideas of memory retrieval and context alignment \citep{godden1975context}. 
\paragraph{}
Overall, memory-inspired architectures and training strategies show strong potential for enhancing LLM performance across various domains, from preventing catastrophic forgetting to increasing the sophistication of counterfactual reasoning. While many of these approaches parallel human cognitive processes—like recalling episodic details or leveraging short-term storage—they also highlight challenges like random memory access and working memory limits. Future research might explore how nuanced schema integration and dynamic memory modules could further align LLM capabilities with the breadth and adaptability of human memory. 

\textbf{Cognitive Development}

\subsection{Cognitive Development}
\label{subsec:cognitive_development}
Cognitive development theories emphasize the gradual changes in human thinking and learning over time. Two influential views include:
\begin{itemize}[nosep,topsep=0pt]
    \item \textbf{Piaget’s Stage Theory:} Describes how children move from basic sensorimotor interactions to more abstract forms of reasoning \citep{piaget1976piaget}.
    \item \textbf{Vygotsky’s Social Interactionism:} Highlights the role of cultural and social frameworks (e.g., scaffolding) in accelerating cognitive growth \citep{Thought and language}.
\end{itemize}

\subsubsection{Stage-Based Learning and Incremental Knowledge Gain}
Building on these theories, researchers propose integrating incremental and real-world tasks into LLM training to mirror children’s progressive learning. \citet{jagadish2024injecting} introduce ecological validity by exposing models to diverse linguistic environments, mimicking how children learn through broad, naturalistic inputs. Similarly, \citet{buschoff2023acquisition} show that stepwise acquisition of physical knowledge mirrors children’s progression from simpler concepts to more advanced ones. \citet{chen-etal-2024-temporal} incorporate constructivist principles, encouraging LLMs to reorganize their understanding based on both correct and incorrect historical samples, a method that resonates with how children adjust their mental models after encountering contradictions \citep{piaget1976piaget}.

\subsubsection{Developmental Alignment and Feedback Loops}
Recent work also highlights parallels between LLM training phases and children’s developmental trajectories. \citet{shah-etal-2024-development} highlight how LLMs exhibit training phases that parallel children’s learning trajectories, suggesting a possible “window of alignment” in which models show the greatest resemblance to human cognitive development. \citet{sharma-etal-2024-laying} emphasize numeracy as an incremental process rooted in real-world distributions, reminiscent of children’s progressive mastery of numerical concepts \citep{piaget1976piaget}. In parallel, \citet{borges-etal-2024-teach} draw on learning science frameworks to introduce structured feedback, echoing Vygotsky’s notion of assisted discovery and scaffolding. Meanwhile, \citet{laverghetta-jr-licato-2022-developmental} connect negation-processing challenges in transformer models to categories from developmental psychology, and \citet{feng-etal-2024-child} investigate child-directed speech for training LLMs, hinting that the child’s data-efficient learning could inspire more effective model training methods. Finally, \citet{sonkar-etal-2023-class} present a scaffolding-based tutoring system, underlining how step-by-step guidance can dynamically shape both student progress and model adaptation \citep{Thought and language}. 
\paragraph{}
By emulating a child’s progression in understanding physical concepts, numerical reasoning, and language structures, LLMs may learn in a more flexible and context-sensitive manner. Nonetheless, open questions remain regarding the optimal “window of alignment” between models and human learners, and the degree to which child-focused data or feedback loops can scale to the complexities of real-world applications. Future work might explore hybrid developmental approaches that combine stage-based tasks with socially oriented scaffolding, ultimately striving for more adaptive and human-aligned language models.


==> cog_dev_papers/data_collection.tex <==
Recent evidence shows that LLMs can align with human brain responses under biologically plausible training conditions \citep{hosseini2024artificial}, despite LLMs typically requiring orders of magnitude more training data than humans receive. This supports the application of \psychTheory{ecological validity} \citep{schmuckler2001ecological} that \psychDef{emphasizes real-world data to mimic cognitive development}. Drawing from this principle, \citet{jagadish2024injecting} selects linguistically diverse environments to reflect children's language acquisition processes, while \citet{feng-etal-2024-child} utilizes child-directed speech to mirror naturalistic learning contexts. In parallel, developmental theories like \psychTheory{incremental numerical understanding} \citep{piaget2013child} view \psychDef{numerical concepts as gradually acquired through exposure} offering insights into sequential data organization. Applying this framework, \citet{sharma-etal-2024-laying} introduces mathematically coherent numeric anchors to align the collection process.


% \paragraph{
%  }
%  One challenge in developing LLMs is their limited ability to generalize across varied real-world contexts, a problem linked directly to ecological validity—a developmental psychology concept emphasizing realistic, context-rich data reflective of human environments. Addressing this,

%Recent evidence shows that LLMs can align with human brain responses under biologically plausible training conditions \citep{hosseini2024artificial}, supporting application of \psychTheory{ecological validity} \citep{schmuckler2001ecological} that \psychDef{emphasizes real-world data to mimic cognitive development}, and \psychTheory{incremental numerical understanding} \citep{piaget2013child} that \psychDef{views numerical concepts as gradually acquired through repeated exposure}.

%  Recent evidence shows that LLMs can align with human brain responses under biologically plausible training conditions \citep{hosseini2024artificial}, despite LLMs typically requiring orders of magnitude more training data than humans receive. This supports the application of \psychTheory{ecological validity} \citep{schmuckler2001ecological} that \psychDef{emphasizes real-world data to mimic cognitive development}. In parallel, developmental theories like \psychTheory{incremental numerical understanding} \citep{piaget2013child} view \psychDef{numerical concepts as gradually acquired through exposure}, offering insights into how data should be sequentially organized for learning.

% To capture ecologically valid datasets, \citet{jagadish2024injecting} selects linguistically diverse environments to reflect language acquisition processes of children. Similarly, \citet{feng-etal-2024-child} utilizes child-directed speech to mirror children's learning. Meanwhile, to enhance numerical understanding, \citet{sharma-etal-2024-laying} introduces mathematically coherent numeric anchors, aligning the collection process with \citet{piaget2013child}. 




==> cog_dev_papers/data_preprocessing.tex <==
%Data preprocessing inspired by cognitive psychology involves refining data to enhance informational coherence prior to training, notably influenced by theories such as \psychTheory{selective attention}\citep{treisman1969selective_attention} that  \psychDef{prioritizes cognitively salient information while filtering out irrelevant stimuli}, and \psychTheory{predictive coding}\citep{rao1999predictive} that proposes \psychDef{anticipatory processing based on prior knowledge}.

Data preprocessing inspired by cognitive psychology involves refining data to enhance informational coherence prior to training. \psychTheory{Selective attention} \citep{treisman1969selective_attention} -- distinct from the attention mechanisms in transformers -- \psychDef{prioritizes cognitively salient information while filtering out irrelevant stimuli}. Implementing this principle, \citet{nottingham-etal-2024-selective} develops a preprocessing model that identifies and filters irrelevant data. Meanwhile, \psychTheory{predictive coding} \citep{rao1999predictive} proposes \psychDef{anticipatory processing based on prior knowledge}, providing a framework for structuring sequential information. Leveraging this insight, \citet{araujo-etal-2021-augmenting} structures sentences to enable anticipation of subsequent content, improving semantic coherence through expectation-driven processing.



% Data preprocessing inspired by cognitive psychology involves refining data to enhance informational coherence prior to training, notably influenced by\psychTheory{selective attention} \citep{treisman1969selective_attention} that \psychDef{prioritizes cognitively salient information while filtering out irrelevant stimuli}--distinct from the attention mechanisms in transformer. Complementing this, \psychTheory{predictive coding} \citep{rao1999predictive} proposes \psychDef{anticipatory processing based on prior knowledge}, providing a framework for structuring sequential information.

% To manage distracting data, \citet{nottingham-etal-2024-selective} applies \psychTheory{selective attention} by implementing a preprocessing model that filters irrelevant data. Additionally, to address semantic incoherence, \citet{araujo-etal-2021-augmenting} embeds \psychTheory{predictive coding} by structuring sentences to enable anticipation of subsequent content, thereby improving semantic coherence.


%{from michelle} It may be more helpful to your audience to explicate the psychological and neuroscience terms since they may not be familiar. Although the link to predictive coding is attractive, I recommend reading this paper as a counterargument: Antonello, R., & Huth, A. G. (2023). Predictive Coding or Just Feature Discovery? An Alternative Account of Why Language Models Fit Brain Data. Neurobiology of Language. https://doi.org/10.1162/nol_a_00087


==> cog_dev_papers/draft.tex <==
% After forming robust foundations with ecologically valid tasks and incremental concept-building in the data and pre-training phase, researchers move on to refine model capabilities especially with theories related to memory structures, attention, and incremental learning. For instance, \cite{deng2024plug} propose a plug-and-play policy planning framework that applies supervised fine-tuning alongside reinforcement learning, showing how children-like iterative feedback helps improve communication strategies. \cite{kang2024think} build on working memory concepts from classic cognitive theories (e.g., Baddeley’s model) by equipping Decision Transformers with a special memory module, mirroring how human learners hold and manipulate information over sequential tasks. \cite{park2024memoria} introduce Memoria, a memory system inspired by multi-store models from developmental psychology (Atkinson and Shiffrin), to address catastrophic forgetting by splitting memory into short-term and long-term parts. \cite{zeng2024framework} extend this idea with a dual-layer memory structure that cooperates with the inference process, capturing the blend of temporary and enduring memory traces often discussed in child cognitive development. Finally, \cite{giannone2024scha} propose a hierarchical approach for few-shot text generation that aggregates context across multiple levels, aligning with schema-based learning theories where knowledge is built up in increasingly complex steps. 


% \textbf{Perception}
% Perception in psychology encompasses a variety of mechanisms, including bottom-up (data-driven) and top-down (knowledge-driven) processes, selective attention, and even subliminal perception—where stimuli below the threshold of conscious awareness can still influence thoughts and behaviors.
% Recent work on perception in LLMs often explores how top-down and bottom-up processes intertwine to create a more coherent understanding of text. \cite{rawte2022tdlr} introduce a framework that prioritizes high-level semantic information before dealing with lower-level syntax, which mirrors top-down processing in human perception, where prior knowledge shapes how we interpret incoming details. \cite{10.5555/3600270.3601883} show that prompting LLMs with “Let’s think step by step” triggers a similar top-down reasoning style. Meanwhile, \cite{araujo-etal-2021-augmenting} adopt predictive coding principles by introducing explicit top-down connections in BERT-style models, allowing the system to anticipate future sentences and adjust its internal representations accordingly. \cite{pang-etal-2023-long}combined bottom-up encoding with top-down corrections to capture both granular details and overarching context. \cite{zhang-etal-2024-holistic} propose Holistic Automated Red Teaming using a top-down approach for test case generation and multi-turn probing, echoing the psychological idea that higher-level strategies can steer how specific inputs are perceived and evaluated.\\ \textbf{Selective Perception} \\ \cite{maharaj-etal-2023-eyes} highlight selective attention by examining users’ gaze behavior for detecting hallucinations, and \emph{Nottingham et al.} take a “selective perception” angle by training a small model to filter out irrelevant input. Their findings about selective attention align with the idea that humans filter complex data by focusing on high-value cues, a hallmark of perceptual processing in psychology. \cite{jung-etal-2024-perceptions} explore “perceptions to beliefs” as precursors to theory of mind, shedding light on how LLMs process initial sensory or textual cues and then infer hidden mental states—a step that parallels how humans form beliefs from raw perceptual data.


% \textbf{Memory}
% In psychology, memory is often dissected into several stages—encoding (taking in information), storage (maintaining it over time), and retrieval (accessing it when needed). Moreover, the concept of working memory highlights our temporary holding and manipulation of data. By aligning these components with LLM design, we can better capture how models handle context and knowledge. \cite{kang2024think} extend Decision Transformers with a working memory module that captures short-term data, reflecting Baddeley’s model of how people hold information “in mind” while performing tasks. \cite{park2024memoria} take this further by adapting Atkinson and Shiffrin’s multi-store concept, splitting memory into short-term and long-term parts and tackles the problem of catastrophic forgetting. \cite{zeng2024framework} propose a dual-layer memory system to balance temporary traces with more enduring information, capturing the interplay of immediate recall and stable knowledge. \cite{giannone2024scha} also touch on memory by applying schema theory that organizes context in layers and gradually build interconnected schemas to interpret information.

% Cognitive development theories—such as Piaget’s stage theory, which stresses progressive learning of concepts, and Vygotsky’s emphasis on social interaction—highlight how human cognition unfolds over time through both incremental knowledge gains and feedback loops. Integrating these insights into LLM training can yield more adaptive, context-aware models. \cite{jagadish2024injecting} underscore ecological validity by injecting training tasks that reflect real-world language use, mimicking children’s natural exposure to diverse situations. \cite{buschoff2023acquisition} show that models can learn physical knowledge incrementally, which parallels how children grasp basic concepts before tackling advanced ones. 

==> language_papers/language.tex <==
The debate over whether large language models (LLMs) possess a true understanding of language or merely function as "stochastic parrots" \citep{10.1145/3442188.3445922} remains ongoing. Linguists have largely been skeptical \citep{AmbridgeBlything20243348}, arguing that language ability is inherently abstract and complex, extending beyond mere statistical pattern recognition. In this survey, we examine recent research on the linguistic capacities of LLMs, covering various aspects of psycholinguistic theory—from word composition to contextual processing.

Human language acquisition exhibits intricate patterns shaped by the interplay of different cognitive faculties. Understanding what LLMs learn—and what they fail to learn—offers valuable insights into the nature of linguistic phenomena and the underlying mechanisms of language processing.

% RQ:

% \begin{itemize}
%     \item General theory Universal Grammar+aspects of linguistic theories
%     \begin{itemize}
%         \item Do LLMs acquire linguistic theories?
%         \item We cannot solve hallucinations, at least certain types of it, without a theory of language or a representation of the language faculty as it is in humans.
%         \item How to learn linguistic theory that is not readily available in the data? Exemplified by the. Cinque hierarchy, raising/control, syntax.
%     \end{itemize}
%     \item Do they share similar “difficulty perceptions” as humans, or similar to child language acquisition?
%     \item Are they able to generalize on “unseen” data? For the mistakes they make, are those different or similar to L2 learners?
% \end{itemize}

% explain what minimal pair is
Methods of studying involves creation of datasets with minimal pairs where one example is grammatical, and the other is ungrammatical with a single difference. ""

\subsection{Language Acquisition}


\psychTheory{Universal Grammar (UG)} \citep{chomsky1957syntactic,chomsky1965aspects} proposes that human brain is innately wired for language, rather than being a blank slate. An apt analogy is a pretrained LLM, which starts with inherent structure rather than learning from scratch. Similarly, the learning patterns of LLMs reflect the patterns of human language acquisition \citep{liu2024zhoblimpsystematicassessmentlanguage}.

% LLMs grasp of Chinese grammar tested against minimal pairs, slightly below human performance on a zero-shot setting. Finetuning reveals a U-shaped learning pattern, similar to child language acquisition \cite{liu2024zhoblimpsystematicassessmentlanguage}.

% competence
Although LLMs have presented near human-level language competence in psycholinguistic tasks \citep{liu2024zhoblimpsystematicassessmentlanguage, duan-etal-2025-unveiling}, identifying lexical semantic equivalence \cite{hayashi-2025-evaluating}, the mechanism to which these models rely on may seem different from the processing mechanisms as humans \citep{lee-etal-2024-psycholinguistic}.

Final-over-Final Condition \cite{Holmberg2000Deriving, sheehan2017fofc} is a proposed syntactic constraint in linguistics that prohibits a head-final phrase from immediately dominating a head-initial phrase within the same extended projection.
\cite{hale-stanojevic-2024-llms} tests LLMs on FOFC linguistic data and found that it was only learned in cases where the model is exposed to developmentally-implausible amounts of training data, but to learn on when the training data size was probably closer to developmental plausibility, such as Basque.


not quite psycholinguistics, but comp ling, 
Word Sense Disambiguation (WSD) 
\cite{kibria-etal-2024-functional} observes that many failure cases are related to a lack of world knowledge and the reasoning to amalgamate this knowledge rather than the lack of linguistic knowledge. 


% Sensitivity to argument roles show that LMs are able to disctinguish verbs that appear in plausible and implausible contexts. none of the models capture the same selective patterns that human comprehenders exhibit during real-time verb prediction. This indicates that language models’ capacity to detect verb plausibility does not arise from the same mechanism that underlies human real-time sentence processing.\cite{lee-etal-2024-psycholinguistic} 

% Using psycholinguistic experiments to investigate LLMs' language competence, showing human level on some tasks \cite{duan-etal-2025-unveiling} % sound-shape association, soundgender association, and implicit causality

\run{check out works by Ev Fedorenko (MIT); Steve Piantadosi (Berkeley). Their work doesnt really concern LLMs, mostly PLMs}

\subsection{Semantics}

\textbf{Conceptual Role Theory} (Harman 1999) \cite{grand2022semantic} \run{Not LLM, but older work that shows LMs may be learning conceptual roles}
\run{Some work laying out LLMs dont work; Roni Katzir (2023), Why large language models are poor theories of human linguistic cognition: A reply to Piantadosi, Biolinguistics, 17(e13153). }
\run{https://arxiv.org/html/2502.07687v1#bib.bib13}
\run{https://www.youtube.com/watch?v=3ZYaxNwHZQo&t=3431s}

\run{https://www.nature.com/articles/s41562-022-01316-8#citeas}

Sample survey paper: \run{https://static1.squarespace.com/static/53d29678e4b04e06965e9423/t/6566e06ac95b0b61f8810a99/1701240942374/2023+--+LLMs+psychology.pdf}; \run{survey of survey: https://github.com/NiuTrans/ABigSurveyOfLLMs}; \run{https://www.nature.com/articles/s44159-023-00241-5};
\run{https://direct.mit.edu/opmi/article/doi/10.1162/opmi_a_00160/124234/The-Limitations-of-Large-Language-Models-for}
\run{https://arxiv.org/html/2409.02387v1}
\\
\run{https://www.nature.com/articles/s42256-024-00976-7}
Research attempts to uncover innate deep structures of language as reflected in the neural architectures of LLMs.

Cross-lingual studies are mixed in terms of linguistic alignment \citep{zhou-etal-2025-linguistic}, although some 

% Linguistic similarity strongly aligns with
% fine-grained theoretical linguistic categories but
% weakly with broader ones. 3) Linguistic similarity shows a weak correlation with semantic
% similarity, showing its context-dependent nature. 4)
% LLMs exhibit limited cross-lingual
% alignment in their understanding of relevant linguistic phenomena
% \cite{zhou-etal-2025-linguistic}

neuron activation patterns of multiligual LLMs show semantic alignment/ language-agnostic activation pattern \cite{zeng-etal-2025-converging}




LLMs latent representations predict human brain activity towards semantic content \cite{nakagi-etal-2024-unveiling}

%QA & evidence selection: LLMs achieve the highest accuracy when the surrounding contexts are composed solely of unrelated information \cite{koo-etal-2024-large}



Additionally, \cite{park-etal-2024-multiprageval} connection
between mathematical reasoning and high-level
linguistic comprehension
\subsection{Pragmatics}
\textbf{Grice’s theory of conversational implicature, Cooperative Principle} interpretation of utterances depends not only on their literal meaning but also, crucially, on
the surrounding context.

\textbf{Harnad's Symbol Grounding Problem (SGP)} posits that for linguistic symbols to be meaningful, they must be grounded in sensory and motor interactions with their referents. %linguistic symbols connect to their non-symbolic referents
\cite{bender-koller-2020-climbing} claims that LLMs cannot really understand linguistic meaning because their symbols are not grounded. On the other hand, \cite{gubelmann-2024-pragmatic} argues that the SGP problem does not apply to LLMs in the context of Theory of Mind.

 The pragmatic performance of LLMs is more closely related to deeper layers than to shallow ones \citep{wu-etal-2024-rethinking}


\textbf{Linguistic Bias} LLMs manifests linguistic discrimination toward speakers of non-”standard” varieties of English \cite{fleisig-etal-2024-linguistic}.
\run{not super relavant in this part, maybe we can disucss the bias in discussions}


\run{not much work on the phonology/phonetics since ALM is quite new, it would be exciting to see the alignment, synergy of the langauge production between different aspsects of language}
% Categorical perception \& language 

% how the contexts inform the linguistic representations of morphemes was exciting for researchers in LM, e.g. embeddings, attention 

% why does the number of tokens per word (?) affect by the training data/LM proficiency

% recurrent/infinite has been solved?






==> language_papers/language_new.tex <==
Evaluation

Psycholinguistic tests have been used to analyze and interpret the language capacity of LLMs. Much of the work evaluates on psycholinguistic tasks, including but not limited to 

In the conversation settings, pragmatics

The LLMs have been 

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> personality/personality.tex <==
% \section{Personality}
Personality research explores the stable patterns of thoughts, feelings, and behaviors that differentiate individuals. Theories of personality generally fall into five major frameworks:

\begin{itemize}[nosep,topsep=0pt]
    \item \textbf{Humanistic Theory:} Emphasizes free will, personal growth, and self-actualization. This perspective focuses on individuals’ subjective experiences and their drive to achieve their full potential \cite{stefaroi2015humanistic}.
    
    \item \textbf{Psychoanalytic Theory:} Originating from Freud, this theory conceptualizes personality as the dynamic interplay between the id, ego, and superego, with unconscious processes playing a central role in shaping behavior.
    
    \item \textbf{Behaviorist Theory:} Views personality as a set of learned responses shaped by environmental reinforcements and punishments. This perspective, pioneered by figures like Skinner and Watson, rejects internal mental states in favor of observable behaviors \cite{pierce2008behavior}.
    
    \item \textbf{Social Cognitive Theory:} Highlights the role of cognitive processes in personality, emphasizing how expectations, beliefs, and observational learning shape behavior \cite{spielman2024psychology}.
    
    \item \textbf{Trait Theory:} Focuses on identifying and measuring stable personality traits that influence behavior across different contexts \cite{cartwright1979theories}.
\end{itemize}

Among these, \textbf{Trait Theory} has been the most widely studied in the context of LLMs, offering insights into how personality can be quantitatively modeled and analyzed.

\subsection{Personality Trait Theory}
Trait theory posits that personality consists of enduring traits that influence behavior. The two most commonly used models in personality research, particularly in the context of AI and LLMs, are the \textbf{Big Five Model} and the \textbf{Myers-Briggs Type Indicator (MBTI)}.

\begin{itemize}[nosep,topsep=0pt]
    \item \textbf{Big Five Model:} The Five-Factor Model (FFM), also known as OCEAN, categorizes personality into five dimensions:
    \begin{itemize}[nosep,topsep=0pt]
        \item \textit{Openness to experience:} Creative, imaginative vs. conventional, routine.
        \item \textit{Conscientiousness:} Organized, responsible vs. careless, impulsive.
        \item \textit{Extraversion:} Sociable, energetic vs. reserved, introverted.
        \item \textit{Agreeableness:} Compassionate, cooperative vs. antagonistic, critical.
        \item \textit{Neuroticism:} Emotionally unstable, anxious vs. calm, resilient \cite{doi:10.1177/0146167202289008}.
    \end{itemize}
    
    \item \textbf{Myers-Briggs Type Indicator (MBTI):} Classifies individuals into 16 personality types based on four dichotomies (e.g., Introversion vs. Extraversion)  \cite{myers1995gifts}. While widely used, MBTI has been criticized for lacking empirical validity, reliability, and independence between its categories \cite{article}. Despite these limitations, MBTI remains influential in corporate and educational settings, with millions of individuals taking the test worldwide.
    \item \textbf{Eysenck Personality Questionnaire-Revised (EPQR-A):} Contains a 24-item personality test that measures extraversion, neuroticism, psychoticism, and social desirability.
\end{itemize}


\subsection{Measuring Personality}

\subsubsection{Measuring User Personality}

NLP research increasingly explores LLMs' ability to infer user personality from text, moving beyond structured psychological tests \cite{rao-etal-2023-chatgpt, yang-etal-2023-psycot} to interactive and multi-agent frameworks \cite{yang-etal-2024-psychogat, yeo-etal-2025-pado}. \cite{rao-etal-2023-chatgpt} developed an MBTI-based evaluation framework, while \cite{yang-etal-2023-psycot} improved Big Five assessments using psychological questionnaire-inspired \textit{Chain-of-Thought} (CoT) prompting. More recent work includes \textbf{PsychoGAT} \cite{yang-etal-2024-psychogat}, which gamifies personality assessments, and \textbf{PADO} \cite{yeo-etal-2025-pado}, a multi-agent framework enhancing contextual inference. Challenges remain in ensuring interpretability, reliability, and applicability across diverse populations, highlighting the need for deeper psychological integration in LLM-driven personality assessment.

% While traditional psychological assessments, such as the Big Five personality traits and MBTI, are well-established, NLP research has increasingly explored the potential of LLMs to infer user personality from text. Initial studies have primarily focused on evaluating LLMs’ ability to assess personality traits using structured psychological tests \cite{rao-etal-2023-chatgpt, yang-etal-2023-psycot}, while more recent efforts integrate interactive methods and multi-agent frameworks to enhance robustness and engagement \cite{yang-etal-2024-psychogat, yeo-etal-2025-pado}.

% Early work examined whether LLMs could function as assessment tools for personality measurement. \cite{rao-etal-2023-chatgpt} proposed a generic framework for using LLMs to complete MBTI tests, introducing unbiased prompts and evaluation metrics to assess consistency and fairness in responses. Similarly, \cite{yang-etal-2023-psycot} demonstrated that structuring personality assessments as psychological questionnaire-inspired \textit{Chain-of-Thought} (CoT) processes improved GPT-3.5’s ability to infer Big Five traits from user text.

% Beyond questionnaire-based methods, recent studies have explored more dynamic approaches to personality assessment. \cite{yang-etal-2024-psychogat} introduced \textbf{PsychoGAT}, which transforms personality assessments into interactive fiction games using LLM agents. Their findings suggest that gamification not only enhances user engagement but also improves psychometric validity. In a different direction, \cite{yeo-etal-2025-pado} developed \textbf{PADO}, a multi-agent framework where multiple LLM-based agents analyze text from different perspectives to infer Big Five personality traits more contextually and robustly.

% Despite these advancements, key challenges remain. Current methods largely focus on text-based self-report assessments, leaving open questions about their applicability across diverse populations and contexts. Additionally, while multi-agent frameworks provide more nuanced personality judgments, their interpretability and reliability require further validation. Future research should explore integrating deeper psychological theories, such as implicit personality constructs, and refining LLM-driven personality inference for real-world applications.

\subsubsection{Measuring Personality Consistency}

Research on personality consistency in LLMs examines whether traits remain stable across interactions and contexts \cite{frisch-giulianelli-2024-llm, amidei-etal-2025-exploring}. \cite{frisch-giulianelli-2024-llm} found that LLMs conditioned on asymmetric personality profiles exhibit varying degrees of consistency in dialogue, highlighting challenges in maintaining stable traits. \cite{amidei-etal-2025-exploring} showed that language switching weakly but significantly alters GPT-4o’s personality expression, reflecting cultural stereotypes. These studies highlight the need for improving personality stability and mitigating biases in LLM-driven interactions.

% \subsubsection{Measuring Personality Consistency}

% The study of personality consistency in LLMs is a rapidly growing area that investigates whether and how LLMs maintain stable personality traits over time and across different contexts. Key studies explore both intra-agent consistency (how a single agent’s personality holds steady during interaction) and inter-agent consistency (how personality traits vary across agents and tasks) \cite{frisch-giulianelli-2024-llm, amidei-etal-2025-exploring}.

% \cite{frisch-giulianelli-2024-llm} examined personality consistency in a population of LLM agents by conditioning GPT-3.5 on asymmetric personality profiles. In their experiments, LLMs were subjected to a collaborative writing task while their responses were evaluated for personality consistency and linguistic alignment. Their findings reveal that different personality profiles exhibit varying levels of consistency in both personality traits and language use, highlighting the challenges of maintaining stable personality expressions in dynamic interaction settings. This work is foundational in exploring how personality can be measured and maintained in LLMs, especially in multi-agent environments.

% Additionally, \cite{amidei-etal-2025-exploring} delved into the impact of language switching on personality consistency. They investigated whether LLMs exhibit personality shifts when switching between languages, using GPT-4o and the Eysenck Personality Questionnaire-Revised (EPQR-A). Their results show that while personality shifts are weak, there is a statistically significant variation in the model’s personality traits across different languages, suggesting that language-switching may influence personality expressions. Furthermore, their study found that GPT-4o reflects distinct country-specific stereotypes when evaluated in different English-speaking regions, emphasizing the potential impact of cultural context on personality consistency in LLMs.

% These studies underscore the importance of examining personality stability in LLMs across different contexts, including multilingual environments and multi-agent interactions. Future research should focus on improving consistency in personality expression, exploring methods to mitigate language-specific or cultural biases, and understanding how such variations affect human-LLM interactions.



% \textbf{Measuring Machine Personality:} With the rise of LLMs, researchers have begun investigating whether personality traits can be meaningfully attributed to AI systems. Approaches include analyzing linguistic patterns, response tendencies, and adaptive behaviors exhibited by LLMs. Studies have explored whether LLMs can be characterized along personality dimensions such as extraversion or agreeableness, and whether such modeling improves user experience and trust \cite{wang2024survey}. 

% Research in this area is ongoing, with debates on whether LLMs truly exhibit personality or merely simulate it through learned patterns. This section explores how personality theories contribute to our understanding of AI behavior and the implications of modeling personality in artificial agents.

\subsubsection{Measuring Machine Personality}

Research on machine personality explores whether LLMs exhibit stable traits and how these can be modified \cite{10.1007/978-981-97-9434-8_19, hu-collier-2024-quantifying}. \cite{10.1007/978-981-97-9434-8_19} introduced \textbf{PersonalityEdit}, a benchmark for systematically adjusting LLM responses to align with \textit{Neuroticism, Extraversion, and Agreeableness}, highlighting challenges in maintaining consistency. \cite{hu-collier-2024-quantifying} examined the \textbf{Persona Effect}, showing that while persona-based prompting improves annotations in ambiguous cases, its impact is limited in most subjective NLP datasets. Future research should refine personality control mechanisms and assess their impact on human-LLM interactions.

While research on human personality assessment using LLMs has gained traction, a parallel line of work explores whether and how personality traits manifest within LLMs themselves. Current studies primarily focus on two areas: \textit{(1) Editing or modifying personality traits in LLMs} to control their responses and \textit{(2) Evaluating the influence of persona-related variables} on LLM behavior \cite{10.1007/978-981-97-9434-8_19, hu-collier-2024-quantifying}.

% Recent work has introduced controlled methods for editing the personality expressions of LLMs. \cite{10.1007/978-981-97-9434-8_19} proposed \textbf{PersonalityEdit}, a benchmark dataset designed to adjust LLM responses to align with specific personality traits. Their study draws from social psychology theories and isolates \textit{Neuroticism, Extraversion, and Agreeableness} as key dimensions. By conditioning GPT-4-generated responses on these traits, they provide insights into how LLM personality expression can be systematically altered. However, challenges remain in ensuring consistent and interpretable personality modifications across different topics and contexts.

% Beyond modifying personality traits, researchers have also investigated how persona-related variables affect LLM outputs. \cite{hu-collier-2024-quantifying} examined the \textbf{Persona Effect}—the extent to which demographic, social, and behavioral variables influence LLM behavior. Their findings indicate that persona variables account for less than 10\% of the variance in existing subjective NLP datasets, but introducing persona-based prompting can still improve LLM-generated annotations in cases with high annotator disagreement. Notably, they identify a linear relationship: the stronger the correlation between persona variables and human annotations, the more effective persona prompting becomes in guiding LLM predictions. However, they also caution that for most subjective datasets, where persona variables have limited explanatory power, the practical benefits of persona prompting remain constrained.

% Despite these developments, research on machine personality is still in its early stages. Open questions remain regarding whether LLMs truly exhibit personality or merely simulate it through learned response patterns. Future directions include refining personality control mechanisms, evaluating stability across different prompts, and investigating whether personality-modulated LLMs lead to improved human-computer interaction outcomes.


\subsection{Modeling Personality in Dialogue}
\textbf{Dialogue Understanding}

Personality traits shape dialogue interactions in LLMs, influencing negotiation and persona-based modeling \cite{huang-hadfi-2024-personality, cheng-etal-2023-marked}. \cite{huang-hadfi-2024-personality} simulated LLM agents with Big Five traits, showing that agreeableness led to better negotiation outcomes while neuroticism resulted in worse ones. \cite{cheng-etal-2023-marked} introduced \textbf{Marked Personas}, revealing biases in LLM-generated personas using a prompt-based method. Their findings highlight concerns over stereotyping in AI-driven dialogue. Future work should refine personality modeling while mitigating biases.

\textbf{Dialogue Generation}

Recent studies have advanced personality-aware dialogue generation by moving beyond static personas, incorporating multimodal empathy, and improving persona consistency \cite{pal-etal-2025-beyond, wu-etal-2025-traits, takayama-etal-2025-persona, chen-etal-2025-comif, ye-etal-2025-sweetiechat}.

\cite{pal-etal-2025-beyond} introduced a dataset of 400K dialogues based on clustered Reddit journal entries, enhancing personality modeling by capturing Big Five traits in generated dialogues. \cite{wu-etal-2025-traits} incorporated multimodal cues (text and images) to generate empathetic responses tailored to user personality. \cite{takayama-etal-2025-persona} improved persona consistency in dialogues using \textbf{Pseudo Preference Tuning}, generating more coherent responses via Direct Preference Optimization (DPO). \cite{chen-etal-2025-comif} proposed \textbf{CoMIF}, a framework that models multiple interaction factors (e.g., personality, emotion, topic) to enhance dialogue realism. \cite{ye-etal-2025-sweetiechat} developed a strategy-enhanced role-playing framework for emotional support agents, refining dialogue adaptation across diverse scenarios.

These approaches push dialogue generation toward more natural, context-aware, and personality-consistent interactions, but challenges remain in balancing multiple personality factors and improving long-term consistency.

% 1. \cite{pal-etal-2025-beyond} Beyond Discrete Personas: Personality Modeling Through Journal Intensive Conversations	COLING 25	Large Language Models (LLMs) have significantly improved personalized conversational capabilities. However, existing datasets like Persona Chat, Synthetic Persona Chat, and Blended Skill Talk rely on static, predefined personas. This approach often results in dialogues that fail to capture human personalities’ fluid and evolving nature. To overcome these limitations, we introduce a novel dataset with around 400,000 dialogues and a framework for generating personalized conversations using long-form journal entries from Reddit. Our approach clusters journal entries for each author and filters them by selecting the most representative cluster, ensuring that the retained entries best reflect the author’s personality. We further refine the data by capturing the Big Five personality traits—openness, conscientiousness, extraversion, agreeableness, and neuroticism—ensuring that dialogues authentically reflect an individual’s personality. Using Llama 3 70B, we generate high-quality, personalityrich dialogues grounded in these journal entries. Fine-tuning models on this dataset leads to an 11% improvement in capturing personality traits on average, outperforming existing approaches in generating more coherent and personality-driven dialogues	Personality Modeling

% 2. \cite{wu-etal-2025-traits}"From Traits to Empathy: Personality-Aware Multimodal Empathetic
% Response Generation"	COLING 25	"Empathetic dialogue systems improve user experience across various domains. Existing approaches mainly focus on acquiring affective
% and cognitive knowledge from text, but neglect the unique personality traits of individuals and the inherently multimodal nature of
% human face-to-face conversation. To this end,
% we enhance the dialogue system1 with the ability to generate empathetic responses from a
% multimodal perspective, and consider the diverse personality traits of users. We incorporate multimodal data, such as images and
% texts, to understand the user’s emotional state
% and situation. "	dialogue generation - empathy

% 3.\cite{takayama-etal-2025-persona} Persona-Consistent Dialogue Generation via Pseudo Preference Tuning	COLING 25	"We propose a simple yet effective method for
% enhancing persona consistency in dialogue response generation using Direct Preference Optimization (DPO). In our method, we generate responses from the response generation model using persona information that has been randomly
% swapped with data from other dialogues, treating these responses as pseudo-negative samples.
% The reference responses serve as positive samples, allowing us to create pseudo-preference
% data. Experimental results demonstrate that
% our model, fine-tuned with DPO on the pseudo
% preference data, produces more consistent and
% natural responses compared to models trained
% using supervised fine-tuning or reinforcement
% learning approaches based on entailment relations between personas and utterances"	dialogue generation

% 4. \cite{chen-etal-2025-comif} CoMIF: Modeling of Complex Multiple Interaction Factors for Conversation Generation	COLING 25	Highly realistic human-machine interaction is challenging for open-domain dialogue systems. Although existing methods have achieved notable progress by leveraging various interaction factors (e.g., emotion, personality, topic) for delivering human-like (e.g., empathetic, personalized and semantically-consistent) responses, they typically model such factors alone and thus easily suffer from low-quality response generation issue, due to the overlook of implicit correlations among factors. Furthermore, different factors may alternately dominate token-level response generation during decoding, making it harder to generate highquality responses by applying various factors at the sentence level. To address the issue, we present a unified response generation framework, which is capable of simultaneously modeling Complex Multiple Interaction Factors (named CoMIF) to generate human-like conversations. To model the implicit correlations among factors, CoMIF first employs a dynamic perception module to construct a directed collaborative-graph to jointly learn the dynamics over time of each factor, as well as the crossdependencies among them. Additionally, we also design a scalable post-adaptation module to introduce token-level factor signals to generate more human-like responses with appropriately multiple factors. Extensive experiments over multiple datasets demonstrate that the proposed method achieves the superior performance in generating more human-like responses with appropriate multiple-factors, as compared to the state-of-the-art methods.	dialogue generation

% 5. \cite{ye-etal-2025-sweetiechat} SweetieChat: A Strategy-Enhanced Role-playing Framework for Diverse Scenarios Handling Emotional Support Agent	COLING 25	To tackle this challenge, we propose an innovative strategy-enhanced role-playing framework, designed to simulate authentic emotional support conversations. Specifically, our approach unfolds in two steps: (1) StrategyEnhanced Role-Playing Interactions, which involve three pivotal roles—Seeker, Strategy Counselor, and Supporter—engaging in diverse scenarios to emulate real-world interactions and promote a broader range of dialogues; and (2) Emotional Support Agent Training, achieved through fine-tuning LLMs using our specially constructed dataset. W	dialogue generation

\subsection{Building Agents with Persona}
\textbf{Dialogue Agents}

Recent work explores persona-driven dialogue agents, focusing on argument generation and personality-based synthetic dialogues \cite{hu-etal-2025-debate, han-etal-2024-psydial}.

\cite{hu-etal-2025-debate} proposed a \textbf{persona-driven multi-agent framework} for argument generation, where agents debate from distinct perspectives to collaboratively construct coherent narratives. This method enhances output diversity and reasoning depth. \cite{han-etal-2024-psydial} introduced \textbf{PSYDIAL}, a personality-based dialogue dataset emphasizing Extraversion from the Big Five model. Their approach improves personality expression in chatbot responses compared to standard models.

These studies highlight the potential of persona-driven frameworks in enhancing dialogue diversity, coherence, and personality alignment.

\textbf{Role-Play Agents}

Recent work has focused on role-playing LLM agents, evaluating their persona alignment, social interaction, and ability to simulate diverse perspectives \cite{castricato-etal-2025-persona, wu-etal-2025-raiden, wang-etal-2025-decoding, chen-etal-2024-socialbench, wang-etal-2024-rolellm, wang-etal-2024-characteristic, mahajan-shaikh-2024-persona, gong2024creamcomparisonbasedreferencefreeeloranked}.

\cite{castricato-etal-2025-persona} introduced \textbf{PERSONA}, a testbed for pluralistic alignment, using 1,586 synthetic personas to evaluate LM responses across diverse user profiles. \cite{wu-etal-2025-raiden} developed the \textbf{RAIDEN Benchmark}, a large-scale dataset assessing role-playing conversational agents (RPCAs) with 40K multi-turn dialogues. \cite{wang-etal-2025-decoding} simulated social opinion networks, modeling echo chambers and polarization using LLM agents. \cite{chen-etal-2024-socialbench} proposed \textbf{SocialBench}, the first benchmark evaluating role-playing agents’ social intelligence at both individual and group levels.

Further, \cite{wang-etal-2024-rolellm} introduced \textbf{RoleLLM}, a framework for benchmarking and fine-tuning role-playing abilities, creating RoleLLaMA and RoleGLM. \cite{wang-etal-2024-characteristic} developed \textbf{Character100}, a dataset for simulating real-life personas in AI agents, enabling systematic evaluation. \cite{mahajan-shaikh-2024-persona} proposed a persona-aware heterogeneous graph transformer to improve response generation in multi-party conversations.

These efforts advance role-playing agents by improving persona consistency, diversity, and realism, though challenges remain in balancing adaptability with coherence in long-term interactions.

% \subsubsection{Role-Play Agents}
% 1. \cite{castricato-etal-2025-persona} PERSONA: A Reproducible Testbed for Pluralistic Alignmen	COLING 25	The rapid advancement of language models (LMs) necessitates robust alignment with diverse user values. However, current preference optimization approaches often fail to capture the plurality of user opinions, instead reinforcing majority viewpoints and marginalizing minority perspectives. We introduce PERSONA, a reproducible test bed designed to evaluate and improve pluralistic alignment of LMs. We procedurally generate diverse user profiles from US census data, resulting in 1,586 synthetic personas with varied demographic and idiosyncratic attributes. We then generate a large-scale evaluation dataset containing 3,868 prompts and 317,200 feedback pairs obtained from our synthetic personas. Leveraging this dataset, we systematically evaluate LM capabilities in role-playing diverse users, verified through human judges, and the establishment of both a benchmark, PERSONA Bench, for pluralistic alignment approaches as well as an extensive dataset to create new and future benchmarks.	role play evaluate pluralistic alignment of LM

% 2. \cite{wu-etal-2025-raiden}RAIDEN Benchmark: Evaluating Role-playing Conversational Agents with Measurement-Driven Custom Dialogues	coling 25	As Large-scale Language Models (LLMs) advance, the development of engaging RolePlaying Conversational Agents (RPCAs) has gained prominence. Despite this progress, there is a notable absence of benchmarks designed around dialogues, rather than questionanswering formats, to assess the effectiveness of RPCA interactions. This paper introduces the RAIDEN benchmark, containing a comprehensive dataset specifically developed for RPCA evaluation, comprising over 40,000 multi-turn utterances across 135 characters. The benchmark focuses on assessing particular dimensions at different stages of a conversation, facilitated through interactions conducted by annotators.	RolePlaying Conversational Agents (RPCAs)

% 3.\cite{wang-etal-2025-decoding} Decoding Echo Chambers: LLM-Powered Simulations Revealing Polarization in Social Networks	coling 25	The impact of social media on critical issues such as echo chambers, needs to be addressed, as these phenomena can have disruptive consequences for our society. Traditional research often oversimplifies emotional tendencies and opinion evolution into numbers and formulas, neglecting that news and communication are conveyed through text, which limits these approaches. Hence, in this work, we propose an LLM-based simulation for the social opinion network to evaluate and counter polarization phenomena. We first construct three typical network structures to simulate different characteristics of social interactions. Then, agents interact based on recommendation algorithms and update their strategies through reasoning and analysis. By comparing these interactions with the classic Bounded Confidence Model (BCM), the Friedkin-Johnsen (FJ) model, and using echo chamber-related indices, we demonstrate the effectiveness of our framework in simulating opinion dynamics and reproducing phenomena such as opinion polarization and echo chambers. We propose two mitigation methods—active and passive nudges—that can help reduce echo chambers, specifically within language-based simulations. We hope our work will offer valuable insights and guidance for social polarization mitigation.1	echo chamber with persona

% 4. \cite{chen-etal-2024-socialbench}SocialBench: Sociality Evaluation of Role-Playing Conversational Agents	ACL 2024 findings	Large language models (LLMs) have advanced the development of various AI conversational agents, including role-playing agents that mimic diverse characters and human behaviors. While prior research has predominantly focused on enhancing the conversational capability, role-specific knowledge and style of these agents, there has been a noticeable gap in assessing their social intelligence. In this paper, we introduce SocialBench, the first benchmark designed to systematically evaluate the sociality of role-playing agents at both individual and group levels of social interactions. SocialBench is constructed from various sources and covers a wide range of 500 characters and over 6,000 question prompts and 30,800 multiturn role-playing utterances. We conducted comprehensive evaluations on this benchmark using mainstream LLMs. We find that agents excelling at the individual level do not necessarily demonstrate proficiency at the group level. Experimental results on SocialBench confirm its significance as a testbed for assessing the social interaction of role-playing agents.	benchmark on role-paly agents

% 5. \cite{wang-etal-2024-rolellm}RoleLLM: Benchmarking, Eliciting, and Enhancing Role-Playing Abilities of Large Language Models	ACL 2024 findings	In this paper, we introduce RoleLLM, a framework to benchmark, elicit, and enhance role-playing abilities in LLMs. RoleLLM comprises four stages: (1) Role Profile Construction for 100 roles; (2) Context-Based Instruction Generation (Context-Instruct) for role-specific knowledge extraction; (3) Role Prompting using GPT (RoleGPT) for speaking style imitation; and (4) Role-Conditioned Instruction Tuning (RoCIT) for fine-tuning open-source models along with role customization. By Context-Instruct and RoleGPT, we create RoleBench, the first systematic and fine-grained character-level benchmark dataset for role-playing with 168,093 samples. Moreover, RoCIT on RoleBench yields RoleLLaMA (English) and RoleGLM (Chinese), significantly enhancing role-playing abilities and even achieving comparable results with RoleGPT (using GPT-4)1	benchmark on role-paly agents

% 6. \cite{wang-etal-2024-characteristic} Characteristic AI Agents via Large Language Models	LREC 24	The advancement of Large Language Models (LLMs) has led to significant enhancements in the performance of chatbot systems. Many researchers have dedicated their efforts to the development of bringing characteristics to chatbots. While there have been commercial products for developing role-driven chatbots using LLMs, it is worth noting that academic research in this area remains relatively scarce. Our research focuses on investigating the performance of LLMs in constructing Characteristic AI Agents by simulating real-life individuals across different settings. Current investigations have primarily focused on act on roles with simple profiles. In response to this research gap, we create a benchmark for the characteristic AI agents task, including dataset, techniques, and evaluation metrics. A dataset called “Character100” is built for this benchmark, comprising the most-visited people on Wikipedia for language models to role-play. With the constructed dataset, we conduct comprehensive assessment of LLMs across various settings. In addition, we devise a set of automatic metrics for quantitative performance evaluation. The experimental results underscore the potential directions for further improvement in the capabilities of LLMs in constructing characteristic AI agents.	dialogue agent

% 7. \cite{mahajan-shaikh-2024-persona}Persona-aware Multi-party Conversation Response Generation	LREC 24	Our main contributions include 1) a multi-party conversation dataset with rich associated metadata (including persona), and 2) a persona-aware heterogeneous graph transformer response generation model. We find that PersonaHeterMPC provides a good baseline towards persona-aware generation for multi-party conversation modeling, generating responses which are relevant and consistent with the interlocutor personas relevant to the conversation.	dialogue agent

\subsubsection{Improve LLMs through persona}

Personality has been used to enhance LLMs in persona consistency, self-improvement, truthfulness, and dialogue coherence.
\cite{jiang-etal-2024-personallm} introduced \textbf{PersonaLLM}, showing that LLMs can generate stable Big Five personality traits, with human evaluators recognizing them with 80\% accuracy. \cite{zhang-etal-2024-self-contrast} proposed \textbf{Self-Contrast}, a method improving LLM reflection by identifying inconsistencies, enhancing response stability. \cite{joshi-etal-2024-personas} introduced the \textbf{Persona Hypothesis}, suggesting LLMs encode truthful and untruthful personas from pretraining data, influencing their truthfulness. \cite{kim-etal-2024-panda} tackled the \textbf{persona overuse problem} in dialogue, developing \textbf{PANDA} to mitigate excessive persona attribution.


\subsection{Reliability of Personality in LLMs}

The reliability of personality in LLMs remains highly debated. Some studies suggest LLMs can consistently simulate personality traits, while others argue that personality assessments applied to these models are unreliable \cite{sorokovikova-etal-2024-llms, gupta-etal-2024-self, shu-etal-2024-dont, huang-etal-2024-reliability, tseng-etal-2024-two}.

\cite{sorokovikova-etal-2024-llms} found that LLaMA-2, GPT-4, and Mixtral exhibit stable Big Five traits, supporting LLMs’ potential for personalized interactions. \cite{huang-etal-2024-reliability} further showed LLMs consistently respond to personality assessments and can emulate diverse personas with prompting.

However, others challenge these findings. \cite{gupta-etal-2024-self} demonstrated that self-assessment tests produce inconsistent results due to prompt sensitivity and response order effects. \cite{shu-etal-2024-dont} further revealed that even minor question variations disrupt LLM personality expression, questioning the validity of these evaluations.

\cite{tseng-etal-2024-two} categorized persona research into \textbf{Role-Playing}, where LLMs adopt assigned personas, and \textbf{Personalization}, where they adapt to users. This distinction raises a fundamental question—do LLMs have inherent personalities, or are they simply reflecting engineered behaviors?

While LLMs may simulate personality, inconsistencies in assessment methods cast doubt on their reliability. Future work may address whether personality in LLMs is emergent or a result of prompt biases.

% The question of whether LLMs truly exhibit stable personality traits or merely simulate them remains a topic of ongoing debate. Some argue that LLMs can consistently reflect personality dimensions, while others highlight the instability and unreliability of personality assessments applied to these models \cite{sorokovikova-etal-2024-llms, gupta-etal-2024-self, shu-etal-2024-dont, huang-etal-2024-reliability, tseng-etal-2024-two}.

% The debate begins with evidence suggesting LLMs can simulate personality traits reliably. \cite{sorokovikova-etal-2024-llms} found that models like LLaMA-2, GPT-4, and Mixtral exhibit stable Big Five personality traits, supporting the idea that LLMs could be used for personalized interactions. \cite{huang-etal-2024-reliability} further reinforced this, showing that LLMs provide consistent responses to personality assessments and can emulate diverse personalities with explicit prompt instructions.

% However, a strong counterargument questions the reliability of personality measurement in LLMs. \cite{gupta-etal-2024-self} demonstrated that self-assessment tests yield highly inconsistent results due to prompt sensitivity and response-order effects, making them unreliable for evaluating LLM personality. Similarly, \cite{shu-etal-2024-dont} found that even minor perturbations in question phrasing significantly affect responses, revealing inconsistencies in LLMs' persona expressions. These results suggest that widely used psychological tools may not translate well to AI models.

% Adding to the complexity, \cite{tseng-etal-2024-two} surveyed research on persona in LLMs, distinguishing between \textbf{LLM Role-Playing}, where models adopt assigned personas, and \textbf{LLM Personalization}, where models cater to user preferences. This highlights a broader issue—whether LLMs exhibit intrinsic personalities or merely reflect engineered behaviors.

% The debate continues: while some see promise in using personality frameworks for LLMs, concerns over reliability and consistency remain unresolved. Future research must determine whether LLM personality is an emergent trait or a reflection of prompt biases, and whether these inconsistencies can be mitigated for more stable, human-like interactions.

==> personality/personalityDebate.tex <==
\textbf{Debates on Reliability of Personality Capability in LLMs}

The reliability of personality in LLMs remains highly debated. Some studies suggest LLMs can consistently simulate personality traits, while others argue that personality assessments applied to these models are unreliable \citep{sorokovikova-etal-2024-llms, gupta-etal-2024-self, shu-etal-2024-dont, huang-etal-2024-reliability, tseng-etal-2024-two}.

\citep{sorokovikova-etal-2024-llms} found that LLaMA-2, GPT-4, and Mixtral exhibit stable \psychTheory{Big Five} traits, supporting LLMs’ potential for personalized interactions. \citep{huang-etal-2024-reliability} further showed LLMs consistently respond to personality assessments and can emulate diverse personas with prompting.

However, others challenge these findings. \citep{gupta-etal-2024-self} demonstrated that self-assessment tests produce inconsistent results due to prompt sensitivity and response order effects. \citep{shu-etal-2024-dont} further revealed that even minor question variations disrupt LLM personality expression, questioning the validity of these evaluations.

\citep{tseng-etal-2024-two} categorized persona research into role-playing, where LLMs adopt assigned personas, and personalization, where they adapt to users. This distinction raises a fundamental question—do LLMs have inherent personalities, or are they simply reflecting engineered behaviors?

While LLMs may simulate personality, inconsistencies in assessment methods cast doubt on their reliability. Future work may address whether personality in LLMs is emergent or a result of prompt biases.

==> post_training/context_retention.tex <==
%Although pre-training equips language models with general knowledge, it falls short in providing context-specific adaptability necessary for specific downstream tasks. SFT Supervised Fine-Tuning (SFT) bridges this gap by explicitly teaching LLMs to better handle and retain context-specific information, aligning responses more closely with downsteam tasks. Specifically, recent work in SFT has begun integrating psychological perspectives, particularly drawing on \psychTheory{Working Memory Theory}, which describes \psychDef{a short-term cognitive system responsible for temporarily holding and manipulating information} \citep{baddeley1974working}. Addressing the critical challenge of context retention in LLMs, \citet{kang2024think} incorporate a dedicated working memory module into Decision Transformers, enabling models to explicitly retain and systematically manage task-relevant short-term information. In contrast, \citet{li-etal-2023-large} propose a more dynamic approach inspired by working memory, introducing methods that adaptively balance newly provided context with previously stored information. These complementary strategies reflect two aspects of working memory—structured retention (Kang) versus dynamic context management (Li).

In SFT, works that draw on psychological insights focus on retaining contextual information. Building on \psychTheory{working memory theory} \citep{baddeley1974working} that proposes \psychDef{a short-term system for temporarily holding information}, \citet{kang2024think} adds a module into Decision Transformers, enabling LLMs to retain and process short-term information. Beyond retaining, \citet{li-etal-2023-large} proposes a working memory approach that dynamically balances stored information with provided contexts for SFT.
% Collectively, these cognitively inspired approaches highlight significant advancements and ongoing challenges in context retention capabilities of LLMs, offering clear benchmarks for future research.

%{michelle} The ways in which working memory is considered have evolved considerably in psychology since the 1970s. It may be worth going beyond merely mentioning working memory as a feature of human memory and explicate the similarities and differences between what Kang and Li contributed with theories. There is also an interesting potential issue of whether LLMs *should* emulate human working memory capacity since it is limited. 


%

==> social/attitude_change.tex <==
\subsection{Attitude Change}
\label{subsec:attitude_change}

Attitude change studies the mechanisms behind shifts in beliefs and attitudes \cite{petty2012communication}. Influential theories in social psychology provide a foundation for understanding persuasion and offer insights that can be leveraged to enhance LLMs. Key theories include:

\begin{itemize}[nosep,topsep=0pt]
    \item \textbf{Cognitive Dissonance Theory:} Explains how inconsistencies between beliefs or behaviors create discomfort, prompting attitude change to restore consistency \cite{morvan2017analysis}.
    \item \textbf{Elaboration Likelihood Model (ELM):} Proposes that persuasion occurs via a central route (deliberate processing) or a peripheral route (heuristic processing), depending on the recipient’s motivation and capacity \cite{petty2012communication}.
    \item \textbf{Balance Theory:} Suggests that individuals strive for consistency among their attitudes and relationships, adjusting beliefs to maintain cognitive harmony \cite{heider1946attitudes}.
    \item \textbf{Inoculation Theory:} Posits that exposure to weak counterarguments can strengthen resistance to persuasion by preemptively activating defensive mechanisms \cite{mcguire1964inducing}.
\end{itemize}

Despite extensive research, little work explicitly evaluates or enhances LLMs using the aforementioned classical attitude change theories. While distinct, these theories collectively address different, fine-grained aspects of persuasion. Most LLM studies apply persuasion models in a task-oriented manner, focusing on, for instance, improving factuality \cite{furumai-etal-2024-zero}, truthfulness \cite{10.5555/3692070.3693020}, and credibility \cite{qin-etal-2024-beyond}, as detailed in Section \ref{subsubsec:persuasion}. Incorporating finer-grained frameworks like ELM or inoculation theory remains an open research area with the potential to enhance collaborative task completion, mitigate biases, and enable LLMs to better simulate the complexities of human persuasion and attitude change.

==> social/group_dynamics.tex <==
\subsection{Group Dynamics}
\label{subsec:group_dynamics}
Group dynamics investigates the behaviors and processes within groups, including conformity and groupthink \cite{tajfel1979integrative, janis1972victims}. These theories offer a insights for improving LLMs' ability to model group interactions, simulate collective decision-making, and navigate social coordination challenges. Influential theories in this area include:

\begin{itemize}[nosep,topsep=0pt]
    % \item \textbf{Social Identity Theory:} Explains how individuals derive their sense of self from group membership, influencing intergroup behavior and social cohesion \cite{tajfel1979integrative}.
    % \item \textbf{Self-Categorization Theory:} Expands on social identity theory, describing how individuals classify themselves and others into social groups, shaping norms and group behaviors \cite{maines1989rediscovering}.
    \item \textbf{Groupthink:} Examines how the desire for conformity and group cohesion can lead to flawed decision-making and suppression of dissenting opinions \cite{janis1972victims}.
    \item \textbf{Social Facilitation and Social Loafing:} Investigates how the presence of others can enhance performance on simple tasks (social facilitation) or reduce effort in collective work (social loafing) \cite{zajonc1965social, latane1979many}.
\end{itemize}

Group dynamics overlaps significantly with several social psychology theories discussed earlier. Many approaches to simulate multi-agent collaboration implicitly address elements of groupthink. For instance, as discussed in Section \ref{subsec:social_influence}, studies explore agents’ ability to simulate human-like collaboration using conformity and collective reasoning \cite{zhang-etal-2024-exploring} or demonstrate how input from users or other agents elicits biases \cite{tjuatja-etal-2024-llms, griffin-etal-2023-large, jin-etal-2024-agentreview}. Similarly, techniques aimed at enhancing collective performance align with social facilitation and social loafing principles. While not explicitly framed in these terms, methods such as task decomposition \cite{wilf-etal-2024-think, jung-etal-2024-perceptions} and perspective modeling \cite{sclar-etal-2023-minding, wang2021tomc, sclar2022symmetric} within multi-agent frameworks enhance ToM capabilities, as detailed in Section \ref{subsubsec:tom}. Likewise, improvements observed in multi-agent debate settings \cite{10.5555/3692070.3693020, rescala-etal-2024-language, liang-etal-2024-encouraging} suggest that the presence of other agents can boost performance on both complex and simple tasks, as discussed in Section \ref{subsubsec:persuasion}. \lin{this section can be further shortened for space, if necessary}

While existing research has simulated groupthink behaviors in LLMs, opportunities remain to directly enhance LLMs to prevent over-groupthinking and mitigate biases. Future research should model additional groupthink elements like obedience and suppression of dissent to improve collective reasoning. Moreover, current multi-agent frameworks are typically tailored to specific tasks; exploring meta-learning strategies or developing a unified paradigm that generalizes across tasks could yield more versatile systems. Integrating these deeper aspects of group dynamics represents a promising direction for advancing the social capabilities of LLMs.

==> social/self_identity.tex <==
\subsection{Self and Identity}
\label{subsec:self_identity}

Self and identity explores the formation of self-concept and social identity \cite{bem1972self, cooley2017human}. These theories can guide the development of LLMs to generate more personalized and context-aware responses by deepening their understanding of self-related concepts. Key theories include:

\begin{itemize}[nosep,topsep=0pt]
    \item \textbf{Self-Perception Theory:} Explains how individuals infer their internal states by observing their own behavior \cite{bem1972self}.
    \item \textbf{Social Identity Theory:} Posits that group membership shapes self-concept and influences intergroup behavior \cite{tajfel1979integrative}.
    \item \textbf{Self-Categorization Theory:} Expands on social identity theory, describing how individuals classify themselves and others into social groups, shaping social norms \cite{maines1989rediscovering}.
    \item \textbf{Self-Discrepancy Theory:} Examines the emotional impact of discrepancies between one’s actual, ideal, and ought selves \cite{higgins1987self}.
    \item \textbf{Self-Affirmation Theory:} Suggests that individuals are motivated to maintain their self-integrity when faced with threats to their self-concept \cite{steele1988psychology}.
    \item \textbf{Symbolic Interactionism:} Emphasizes that the self is constructed through social interactions and the use of symbols, such as language \cite{blumer1986symbolic}.
\end{itemize}

Although our review finds limited work explicitly applying self and identity theories to LLMs, a closely related and growing area of research involves self-reflective mechanisms. Self-reflection -- where a model evaluates its outputs to update internal ``beliefs” and improve performance -- conceptually aligns with theories like self-perception and self-affirmation, which emphasize introspection and self-assessment in shaping self-concept.

\subsubsection{Self-Reflective Mechanisms}
\label{subsubsec:self_reflect}
Self-reflective methods have been applied across various tasks, including hallucination mitigation and factuality improvement \cite{ji-etal-2023-towards}, machine translation \cite{chen-etal-2024-dual, wang-etal-2024-taste}, question answering \cite{li-etal-2024-hindsight, zhang-etal-2024-learn, kassner-etal-2023-language}, mathematical reasoning \cite{zhang-etal-2024-learn}, and named entity recognition \cite{heng-etal-2024-proggen}. \textbf{Multi-agent frameworks}, such as reflective collaboration \cite{NEURIPS2024_fa54b0ed} and hierarchical agents \cite{pmlr-v235-du24h}, extend these techniques to collective environments.

Several methods adopt dual or multi-step reflection processes \cite{li-etal-2024-think}, where iterative self-reflection \cite{ji-etal-2023-towards, yan-etal-2024-mirror} and task decomposition \cite{wang-etal-2024-taste, zhang-etal-2024-self-contrast} refine intermediate reasoning steps, improving factuality and reducing hallucinations. Reinforcement learning (RL) further optimizes self-reflection, as seen in reflection-reinforced self-training \cite{dou-etal-2024-rest}, confidence-calibrating reward functions \cite{xu-etal-2024-sayself}, and semantic memory-augmented RL \cite{gupta-etal-2024-metareflection}, which enhance task performance. Additionally, self-reflective rationales \cite{kassner-etal-2023-language, ramnath2024tailoring} and uncertainty-aware methods \cite{zhao-etal-2024-fact, NEURIPS2024_b130a569} help calibrate confidence levels, though studies indicate that LLM self-explanations are not always reliable \cite{madsen-etal-2024-self}.

These methods collectively demonstrate that self-reflection can improve consistency, reasoning, and calibration across diverse tasks. While their connection to self and identity theories is indirect, they align with the core idea that introspection and self-assessment drive continuous improvement. Future research should explore unified frameworks that integrate these techniques and more explicitly align them with self and identity constructs, potentially enabling LLMs to exhibit more human-like behaviors and understand social norms and nuances. Additionally, theories such as self-identity, self-discrepancy, and self-affirmation present promising avenues for enhancing LLMs’ ability to model human behavior and complex social interactions.

==> social/social.tex <==
Social psychology encompasses key areas such as \textit{Social Cognition} \cite{fiske2020social, baron2012science}, \textit{Social Influence} \cite{cialdini2009influence, milgram1963behavioral}, \textit{Group Dynamics} \cite{tajfel1979integrative, janis1972victims}, \textit{Attitude Change} \cite{petty2012communication}, and \textit{Self and Identity} \cite{bem1972self, cooley2017human}. With the rise of LLMs, these theories provide a strong foundation for developing socially intelligent AI, enhancing their ability in:

\begin{itemize}[nosep,topsep=0pt]
    \item \textbf{Modeling Human-Like Behavior:} Social psychology aids the design of LLMs that exhibit human-like empathy, adapt to users' emotions, and engage in nuanced conversations \cite{wang2024survey, wang2025limits}.
    
    \item \textbf{Adaptive and Contextual Interaction:} Concepts like theory of mind help LLMs infer and respond to users' mental states, enabling more natural, context-aware interactions \cite{wilf2023think, zhang-etal-2024-exploring}.
    
    \item \textbf{Bias Mitigation and Ethical Alignment:} Theories of attitude change and social influence guide to bias reduction, ensuring responsible responses \cite{kamruzzaman2024prompting, raj2024breaking, tjuatja-etal-2024-llms}.
\end{itemize}

Research on LLMs' social capabilities primarily falls into two domains: \textbf{(a) Interpersonal Interaction:} One-on-one exchanges where LLMs build rapport, foster trust, and demonstrate social sensitivity; and \textbf{(b) Group Dynamics:} Multi-agent settings where LLMs must navigate complex social processes such as consensus-building and conflict resolution. This section examines how theories from social psychology enhance LLMs' performance across these domains.

% \subsection{Social Psychology Areas}
% Social psychology encompasses a wide range of theories and influential areas, including
% \begin{itemize}[nosep,topsep=0pt]
%     \item \textbf{Social Cognition:} Focuses on how individuals perceive and interpret social information \cite{fiske2020social, baron2012science}.
%     \item \textbf{Social Influence:} Examines how individuals are affected by the behaviors and opinions of others \cite{cialdini2009influence, milgram1963behavioral}.
%     \item \textbf{Group Dynamics:} Investigates the behaviors and processes within groups, including conformity and groupthink \cite{tajfel1979integrative, janis1972victims}.
%     \item \textbf{Attitude Change:} Studies the mechanisms behind shifts in beliefs and attitudes \cite{petty2012communication}.
%     \item \textbf{Self and Identity:} Explores the formation of self-concept and social identity \cite{bem1972self, cooley2017human}.
% \end{itemize}


\begin{comment}
1.	Social Cognition:
	•	Attribution Theory: Explores how people explain the causes of behavior, distinguishing between internal (dispositional) and external (situational) factors.
	•	Schema Theory: Focuses on the mental frameworks or schemas that help individuals organize and interpret information.
	•	Dual-Process Models: Such as Kahneman’s System 1 (fast, intuitive) and System 2 (slow, deliberate), which explain how social judgments and decisions are made.
	•	Theory of Mind: Involves the ability to infer others’ mental states, beliefs, and intentions.
	2.	Social Influence:
	•	Social Impact Theory: Proposes that the impact of social influence depends on the strength, immediacy, and number of sources.
	•	Conformity Theories: Based on studies by Asch, these theories explain how group pressure can lead individuals to conform to majority opinions.
	•	Obedience Theories: Exemplified by Milgram’s work, focusing on how authority influences individuals’ compliance.
	•	Persuasion Models: Such as the Elaboration Likelihood Model (ELM) and the Heuristic-Systematic Model, which explain the routes through which persuasive messages influence attitudes.
	3.	Group Dynamics:
	•	Social Identity Theory: Explains how group membership influences self-concept and behavior, highlighting in-group vs. out-group dynamics.
	•	Self-Categorization Theory: A complement to Social Identity Theory, focusing on how people classify themselves and others into groups.
	•	Groupthink: Describes how the desire for group cohesion can lead to poor decision-making.
	•	Social Facilitation and Social Loafing: Address how the presence of others can enhance or diminish individual performance within groups.
	4.	Attitude Change:
	•	Cognitive Dissonance Theory: Festinger’s theory which states that individuals experience discomfort when holding conflicting attitudes, prompting a change to reduce the dissonance.
	•	Elaboration Likelihood Model (ELM): Describes how persuasion occurs via a central (logic-based) or peripheral (emotion/heuristic-based) route.
	•	Balance Theory: Suggests that people strive for harmony in their relationships and attitudes, leading to attitude adjustments to resolve inconsistencies.
	•	Inoculation Theory: Proposes that exposure to weakened counterarguments can build resistance to persuasion.
	5.	Self and Identity:
	•	Self-Perception Theory: Bem’s idea that people infer their own attitudes and feelings by observing their behavior.
	•	Social Identity Theory and Self-Categorization Theory: Highlight how identification with social groups shapes self-concept and influences behavior.
	•	Self-Discrepancy Theory: Higgins’ theory focusing on the differences between one’s actual, ideal, and ought selves, which can affect emotions and motivation.
	•	Self-Affirmation Theory: Steele’s theory suggesting that people are motivated to maintain their self-integrity, which influences how they process information about themselves.
	•	Symbolic Interactionism: Emphasizes the role of social interactions and the use of symbols (such as language) in the formation of the self.
\end{comment}

\input{social/social_cognition}
\input{social/social_influence}
\input{social/group_dynamics}
\input{social/attitude_change}
\input{social/self_identity}

==> social/social_cognition.tex <==
\subsection{Social Cognition}
\label{subsec:social_cognition}
Social cognition focuses on how individuals perceive and interpret social information \cite{fiske2020social, baron2012science}. Research in social cognition offers a robust framework for understanding how humans perceive, interpret, and respond to social information. Key theories include:
\begin{itemize}[nosep,topsep=0pt]
    \item \textbf{Attribution Theory:} Explains how people infer causes of behavior as internal (dispositional) or external (situational) \cite{fiske2020social, baron2012science}.
    \item \textbf{Schema Theory:} Focuses on mental frameworks (schemas) that organize and guide interpretation of information \cite{rumelhart2017schemata, frith2008social}.
    \item \textbf{Dual-Process Models:} Differentiate between fast, intuitive (System 1) and slow, deliberate (System 2) processing in social judgment, inspiring LLM reasoning enhancements \cite{kahneman2011thinking}.
    \item \textbf{Theory of Mind (ToM):} Refers to the ability to infer others’ mental states, crucial for social interaction \cite{baron1985does}.
\end{itemize}
Many recent approaches draw inspiration, particularly from dual-process models and ToM.

\subsubsection{Dual-Process Models}
\label{subsubsec:dual_process}
Dual-process models, which separate fast, intuitive from slow, deliberate reasoning, offer a promising framework for enhancing LLM performance. For instance, chain-of-thought prompting \cite{wei2022chain} encourages the model to generate intermediate reasoning steps, effectively engaging System 2 processes and improving performance on complex tasks. Building on this, the DynaThink framework \cite{pan-etal-2024-dynathink} enables LLMs to dynamically select between rapid and thorough inference based on task complexity. Additionally, the Tree of Thoughts approach \cite{yao2024tree} allows the exploration of multiple reasoning paths concurrently, further refining deliberative processing. Together, these methods not only reduce errors and enhance decision-making but also open avenues for future research, such as integrating reinforcement learning for dynamic task routing and improving long-horizon context management.

% \subsubsection{ToM}
% \label{subsubsec:tom}
% Integrating ToM into LLMs is a promising avenue for enhancing their social cognition. ToM refers to the ability to infer others’ beliefs, desires, and intentions—a critical faculty for effective social interaction \cite{baron1985does}. Recent research in this area can be broadly categorized into two themes: \textbf{(1)} Evaluation and benchmarking of ToM capabilities in LLMs and \textbf{(2)} Model enhancement approaches that incorporate explicit ToM mechanisms, with further distinctions between methods for interpersonal interactions and group dynamics.

% A number of studies have focused on establishing comprehensive benchmarks and evaluation protocols. For example, \textit{ToMBENCH} \cite{chen-etal-2024-tombench} and \textit{OpenToM} \cite{xu-etal-2024-opentom} introduce datasets featuring longer narratives, explicit personality traits, and action-triggered questions, specifically designed to test LLMs’ ability to model mental states in both interpersonal and group contexts. Similarly, \textit{HI-TOM} \cite{wu-etal-2023-hi} targets higher-order ToM reasoning by evaluating recursive inference of beliefs, while \textit{FANTOM} \cite{kim-etal-2023-fantom} stresses models in information-asymmetric conversational settings. The dataset \textit{Views Are My Own, but Also Yours} \cite{soubki-etal-2024-views} further addresses natural dialog-based interactions by grounding evaluation in spoken conversation, highlighting persistent performance gaps relative to human benchmarks. In addition, position and survey papers \cite{ma-etal-2023-towards-holistic, sap-etal-2022-neural} provide valuable taxonomies and discuss the limitations of current approaches.

% On the model enhancement side, several works incorporate explicit ToM mechanisms to improve reasoning. In \textbf{interpersonal settings}, approaches show that integrating ToM features can improve missing knowledge prediction \cite{bortoletto-etal-2024-limits} and common ground alignment and negotiation \cite{qiu-etal-2024-minddial} in dialogue-based tasks. \citet{wu-etal-2024-coke}  formalize cognitive
% processes as a chained structure, enhancing LLMs' ToM ability in social applications. For \textbf{multi-agent settings}, methods such as \citet{sclar-etal-2023-minding} enable LLMs to track multiple characters’ beliefs in reading comprehension tasks. \citet{wang2021tomc, sclar2022symmetric} introduce frameworks where agents use local observations to infer others’ mental states and coordinate actions in tasks like cooperative navigation. Moreover, \citet{sileo-lernould-2023-mindgames} leverages dynamic epistemic modal logic to isolate components of ToM and generate controlled problems, revealing that increasing model scale does not always yield proportional gains in epistemic reasoning. Finally, approaches such as \citet{wilf-etal-2024-think, jung-etal-2024-perceptions} adopt simulation and perspective-taking frameworks (inspired by dual-process and Simulation Theory) to decompose complex ToM tasks into simpler subtasks (e.g., subject identification, question reframing, world model updating). \citet{sarangi-etal-2025-decompose} further refines this by recursively simulating user perspectives.

% Interesting findings across these studies include consistent evidence that even state-of-the-art LLMs (e.g., GPT-4) lag behind human performance by over 10\% on many ToM benchmarks, as well as challenges such as long-horizon context management and hallucination of task states. Future opportunities lie in integrating reinforcement learning with explicit ToM representations, developing more robust cross-domain benchmarks, and exploring hybrid neural-symbolic models to further narrow the performance gap. Collectively, these efforts demonstrate the potential of ToM-inspired approaches to endow LLMs with richer, more human-like social cognition, ultimately improving both individual and group interactions.

\subsubsection{ToM}
\label{subsubsec:tom}
Integrating ToM into LLMs enhances their ability to infer beliefs, desires, and intentions, crucial for social interaction \cite{baron1985does}. Recent research focuses on two areas: \textbf{(1)} evaluation and benchmarking, and \textbf{(2)} model enhancements for interpersonal and multi-agent interactions.

For evaluation, benchmarks like \textit{ToMBENCH} \cite{chen-etal-2024-tombench} and \textit{OpenToM} \cite{xu-etal-2024-opentom} assess LLMs on mental state modeling, while \textit{HI-TOM} \cite{wu-etal-2023-hi} and \textit{FANTOM} \cite{kim-etal-2023-fantom} test higher-order reasoning and asymmetric information scenarios. \citet{soubki-etal-2024-views} extend ToM evaluation to spoken dialogues, highlighting gaps between LLM and human performance. Surveys \cite{ma-etal-2023-towards-holistic, sap-etal-2022-neural} outline existing challenges and research directions.

For model enhancements, \textbf{interpersonal methods} improve missing knowledge inference \cite{bortoletto-etal-2024-limits}, common ground alignment \cite{qiu-etal-2024-minddial}, and cognitive modeling \cite{wu-etal-2024-coke}. \textbf{Multi-agent approaches} enable characters' belief tracking \cite{sclar-etal-2023-minding} and coordination in social tasks \cite{wang2021tomc, sclar2022symmetric}. Logic-based frameworks \cite{sileo-lernould-2023-mindgames} show that increasing model scale does not always enhance epistemic reasoning. Inspired by dual-process and Simulation Theory, strategies \cite{wilf-etal-2024-think, jung-etal-2024-perceptions} refine ToM capabilities through task decomposition, further extended by recursive simulations \cite{sarangi-etal-2025-decompose}.

Findings show that even advanced LLMs underperform humans by over 10\% on many ToM tasks, struggling with long-horizon contexts and hallucinations. Future work should integrate reinforcement learning, improve cross-domain benchmarks, and explore hybrid neural-symbolic models to advance ToM reasoning in LLMs. 

==> social/social_influence.tex <==
\subsection{Social Influence}
\label{subsec:social_influence}

Social influence examines how individuals are affected by the behaviors and opinions of others \cite{cialdini2009influence, milgram1963behavioral}. Insights from this field can be leveraged to enhance LLMs by improving their sensitivity to subtle social cues, mitigating biases, and advancing their ability to interpret group dynamics.
Influential theories in this area include:

\begin{itemize}[nosep,topsep=0pt]
    \item \textbf{Social Impact Theory:} This theory posits that the magnitude of social influence depends on the strength, immediacy, and number of sources \cite{latane1981psychology}.
    \item \textbf{Conformity Theories:} Based on seminal work by Asch, these theories explore how group pressure can alter individual judgments \cite{asch2016effects}.
    \item \textbf{Obedience Theories:} Milgram’s studies demonstrate how authority influences behavior, highlighting conditions under which individuals comply \cite{milgram1963behavioral}.
    \item \textbf{Persuasion Models:} The Elaboration Likelihood Model explains how messages processed via central or peripheral routes can lead to attitude change \cite{petty2012communication}.
\end{itemize}

In general, social influence theories remain largely underexplored in enhancing LLMs. Some studies examine LLM-based agents’ ability to simulate human-like collaboration using psychological principles like conformity and collective reasoning \cite{zhang-etal-2024-exploring}, while others analyze response biases to prompt variations \cite{tjuatja-etal-2024-llms, griffin-etal-2023-large} or input from other agents \cite{jin-etal-2024-agentreview}. However, integrating theories such as obedience remains a gap. Moreover, although much research has evaluated LLMs on broader social influence issues, including gender biases \cite{oba-etal-2024-contextual, zhao-etal-2024-comparative}, social biases \cite{shin-etal-2024-ask, lee-etal-2023-kosbi, nozza-etal-2022-pipelines}, and stereotypes \cite{shrawgi-etal-2024-uncovering, huang-xiong-2024-cbbq, grigoreva-etal-2024-rubia}, direct applications of social influence theories -- such as social impact theory -- for bias mitigation or agent responsiveness remain an open research area. Therefore, this section primarily discusses work integrating persuasion models in LLM applications.

\subsubsection{Persuasion Models}

\label{subsubsec:persuasion}
% Persuasion models offer valuable insights into how language and behavior can be shaped to influence attitudes and decisions. In the \textbf{interpersonal interaction applications}, several studies have designed persuasive chatbots and conversational recommender systems. For instance, \citet{gollapalli-ng-2025-pirsuader} leverage a context-specific persuasive dialog act schema and reinforcement learning to mitigate psychological insulin resistance in type-2 diabetic patients, while\citet{furumai-etal-2024-zero} combine LLM-generated strategies with information retrieval to improve factuality and persuasiveness. Similarly, \citet{qin-etal-2024-beyond} and \citet{jin-etal-2024-persuading} introduce methods that guide explanation generation via credibility-aware strategies and intent-to-strategy reasoning, respectively. A distinct line of inquiry is presented by \citet{zeng-etal-2024-johnny}, which applies a persuasion taxonomy to generate adversarial prompts that expose vulnerabilities in LLMs, highlighting the need for robust defenses.

% In \textbf{multi-agent or group settings}, persuasion models have been applied to simulate negotiation and debate scenarios. \citet{huang-hadfi-2024-personality} use a simulation framework where LLM agents with synthesized personality traits negotiate, reproducing behavioral patterns observed in human negotiations. Additionally, \citet{10.5555/3692070.3693020} demonstrates that structuring debates between LLM experts can significantly boost the truthfulness of responses, \citet{rescala-etal-2024-language} extend existing datasets to assess LLMs’ ability to distinguish strong from weak arguments, with ensemble predictions surpassing human performance.

% Overall, these studies reveal promising improvements -- such as enhanced persuasive effectiveness, more credible explanations, and better alignment of negotiation outcomes -- while also exposing challenges like long-horizon context management and increased jailbreak risks. Future opportunities lie in integrating reinforcement learning with dynamic persuasive strategies, expanding multi-domain datasets, and developing hybrid models that combine neural and symbolic approaches to further refine the social influence capabilities of LLMs.
% \gary{i feel like my style of writing are mostly like this paragraph. section 8.2 and 8.1 seems like two different way of telling stories. We should discuss which way do we want to go with for consistency?}
Persuasion models provide insights into shaping language and behavior to influence attitudes and decisions. In \textbf{interpersonal interactions}, studies have developed persuasive chatbots and recommender systems. \citet{gollapalli-ng-2025-pirsuader} employ a persuasive dialog act schema and reinforcement learning to mitigate psychological insulin resistance, while \citet{furumai-etal-2024-zero} integrate LLM-generated strategies with retrieval to enhance factuality and persuasiveness. Similarly, \citet{qin-etal-2024-beyond} and \citet{jin-etal-2024-persuading} guide explanation generation using credibility-aware strategies and intent-to-strategy reasoning. \citet{zeng-etal-2024-johnny} take a different approach, applying a persuasion taxonomy to generate adversarial prompts, exposing LLM vulnerabilities.

In \textbf{multi-agent settings}, persuasion models facilitate negotiation and debate simulations. \citet{huang-hadfi-2024-personality} use synthesized personality traits to model LLM-based negotiations, mirroring human behaviors. \citet{10.5555/3692070.3693020} demonstrate that structured debates between LLM experts improve truthfulness, while \citet{rescala-etal-2024-language} extend datasets to assess argument strength, with ensemble models outperforming human evaluation.

These studies show advancements in persuasive effectiveness, credibility, and negotiation alignment, but challenges remain, such as long-horizon context management and jailbreak risks. Future directions include integrating reinforcement learning and multi-domain datasets to enhance LLMs' social influence capabilities.

